Revisiting Local PageRank Estimation on Undirected Graphs: Simple and Optimal

We propose a simple and optimal algorithm, BackMC, for local PageRank estimation in undirected graphs: given an arbitrary target node $t$ in an undirected graph $G$ comprising $n$ nodes and $m$ edges, BackMC accurately estimates the PageRank score of node $t$ while assuring a small relative error and a high success probability. The worst-case computational complexity of BackMC is upper bounded by $O\left(\frac{1}{d_{\mathrm{min}}}\cdot \min\left(d_t, m^{1/2}\right)\right)$, where $d_{\mathrm{min}}$ denotes the minimum degree of $G$, and $d_t$ denotes the degree of $t$, respectively. Compared to the previously best upper bound of $ O\left(\log{n}\cdot \min\left(d_t, m^{1/2}\right)\right)$ (VLDB '23), which is derived from a significantly more complex algorithm and analysis, our BackMC improves the computational complexity for this problem by a factor of $\Theta\left(\frac{\log{n}}{d_{\mathrm{min}}}\right)$ with a much simpler algorithm. Furthermore, we establish a matching lower bound of $\Omega\left(\frac{1}{d_{\mathrm{min}}}\cdot \min\left(d_t, m^{1/2}\right)\right)$ for any algorithm that attempts to solve the problem of local PageRank estimation, demonstrating the theoretical optimality of our BackMC. We conduct extensive experiments on various large-scale real-world and synthetic graphs, where BackMC consistently shows superior performance.

==> analysis.tex <==
\section{Theoretical Analysis}
\label{sec:analysis}
In this section, we analyze the theoretical properties of the \setpush algorithm. First, we formally prove that the $\ell$-hop residue $\r^{(\ell)}_t(u)$ is an unbiased estimator of $\frac{1}{\alpha}\vpi^{(\ell)}_t(u)$, and the output $\epi(t)$ returned by Algorithm~\ref{alg:VBES} is an unbiased estimator of the truncated PageRank $\bpi(t)$. Then Section~\ref{subsec:variance} provides the bound of the variance of $\epi(t)$. Finally, in Section~\ref{subsec:totalcost}, Theorem~\ref{thm:finalcost_analysis} presents the theoretical guarantees and expected time cost of the \setpush algorithm. 


\subsection{Correctness}\label{subsec:correctness}
Recall that we given some intuitions for $\E\left[\r^{(\ell)}_t(u)\right]=\frac{1}{\alpha}\vpi^{(\ell)}_t(u)$ in Section~\ref{subsec:highlevelidea}. In the following, Lemma~\ref{lem:unbiasedness_er} provides a formal proof of this observation. 

\begin{lemma}\label{lem:unbiasedness_er}
The residue vector $\er^{(\ell+1)}_t$ obtained by Algorithm~\ref{alg:VBES} in the $(\ell+1)$-th iteration is an unbiased estimator of $\frac{1}{\alpha}\vpi^{(\ell+1)}_t$ such that 
\begin{align*}
\E \left[\er^{(\ell+1)}_t(v)\right]=\frac{1}{\alpha}\cdot \vpi^{(\ell+1)}_t(v)    
\end{align*}
holds for $\forall v\in V$ and $\forall \ell\in \{0,1, \ldots, L-1\}$. 
\end{lemma}

\begin{proof}
Let $\incre^{(\ell+1)}(u,v)$ denote the probability mass transferred from node $u$ to node $v$ in the $(\ell+1)$-th iteration of Algorithm~\ref{alg:VBES}. According to Algorithm~\ref{alg:VBES}, in the $(\ell+1)$-th iteration with the derived estimator $\er^{(\ell)}_t$, we deterministically set $\incre^{(\ell+1)}(u,v)=\frac{1-\alpha}{d_u}\cdot \er^{(\ell)}_t(u)$ if $\frac{(1-\alpha)}{d_u}\cdot \er^{(\ell)}_t(u)\ge \th$. Otherwise, we set $\incre^{(\ell+1)}(u,v)=\th$ with probability $\frac{(1-\alpha)}{d_u \cdot \th}\cdot \er^{(\ell)}_t(u)$, leading to the expectation of $\incre^{(\ell+1)}(u,v)$ as $\th \cdot \frac{(1-\alpha)}{d_u \cdot \th}\cdot \er^{(\ell)}_t(u)=\frac{(1-\alpha)}{d_u}\cdot \er^{(\ell)}_t(u)$. As a result, 
\begin{align*}
\E \left[\incre^{(\ell+1)}(u,v) \mid \er^{(\ell)}_t\right]=\frac{(1-\alpha)}{d_u}\cdot \er^{(\ell)}_t(u). 
\end{align*}
always holds after the $(\ell+1)$-th iteration. Furthermore, since $\er^{(\ell)}(v)=\sum_{u\in N(v)}\incre^{(\ell+1)}(u,v)$, we can derive: 
\begin{align}\label{eqn:conditional_exp}
\E \left[\er^{(\ell+1)}_t(v)~\big|~\er^{(\ell)}_t\right]\hspace{-1mm}=\hspace{-3mm}\sum_{u\in N(v)}\hspace{-3mm}\E \left[\incre^{(\ell+1)}(u,v) ~\big|~\er^{(\ell)}_t\right]\hspace{-1mm}=\hspace{-3mm}\sum_{u\in N(v)}\hspace{-3mm}\frac{(1-\alpha)}{d_u}\hspace{-0.5mm}\cdot \hspace{-0.5mm}\er^{(\ell)}_t(u)
\end{align}
by applying the linearity of expectation. Given the fact: $\E[\er^{(\ell+1)}(v)]=\E\left[ \E \left[\er^{(\ell+1)}(v)~\big|~\er^{(\ell)}_t\right]\right]$, we can further derive: 
\begin{align}\label{eqn:recur_er}
\E \left[\er^{(\ell+1)}(v)\right]=\sum_{u\in N(v)}\frac{(1-\alpha)}{d_u}\cdot \E\left[\er^{(\ell)}_t(u)\right].
\end{align}
Based on the recursive formula as shown in Equation~\eqref{eqn:recur_er}, we are able to prove Lemma~\ref{lem:unbiasedness_er} by mathematical induction. Specifically, the base case $\er^{(0)}_t=\bm{e}_s=\frac{1}{\alpha}\cdot \vpi^{(0)}_t$ holds according to Algorithm~\ref{alg:VBES}. For the inductive case, assuming that $\E\left[\er^{(\ell)}_t(u)\right]=\frac{\vpi^{(\ell)}_t(u)}{\alpha}$ holds for each $u\in V$, by Equation~\eqref{eqn:recur_er}, we have:   
\begin{align*}
\E\left[\er^{(\ell+1)}_t(v)\right]\hspace{-1mm}=\hspace{-1mm}\frac{1}{\alpha}\cdot \hspace{-2mm}\sum_{u\in N(v)}\hspace{-1mm}\frac{(1-\alpha)}{d_u}\cdot \vpi^{(\ell)}_t(u)=\frac{1}{\alpha}\cdot \vpi^{(\ell+1)}_t(v),  
\end{align*}
where we apply the fact that $\vpi^{(\ell+1)}_t(v)=\sum_{u\in N(v)}\frac{(1-\alpha)}{d_u}\cdot \vpi^{(\ell)}_t(u)$ given in Equation~\eqref{eqn:PPR_recur}. Consequently, the inductive case holds, and Lemma~\ref{lem:unbiasedness_er} follows. 
\end{proof}

Based on Lemma~\ref{lem:unbiasedness_er}, we are able to prove that Algorithm~\ref{alg:VBES} returns an unbiased estimator of the truncated PageRank $\bpi(t)$. 

\begin{lemma}\label{lem:unbiasedness_ppr}
%For each node $s\in V$, Algorithm~\ref{alg:VBES} computes an estimator $\epi_t(s)$ such that $\E[\epi_t(s)]=\bpi_t(s)$. 
Algorithm~\ref{alg:VBES} returns an unbiased estimator $\epi(t)$ for the truncated PageRank of node $t$, such that $\E[\epi(t)]=\bpi(t)$. 
\end{lemma}
\begin{proof} 
Recall that after the $(\ell+1)$-th iteration of Algorithm~\ref{alg:VBES}, we update $\epi_t$ by $\epi_t+\alpha \er^{(\ell+1)}_t$, and initially $\epi_t$ is set as $\alpha \bm{e}_s$. Thus, for each node $s\in V$, $\epi_t(s)=\sum_{\ell=0}^{L} \alpha \cdot \er^{(\ell)}_t(s)$. Furthermore, we compute $\epi(t)=\frac{1}{n}\cdot \sum_{s\in V}\frac{d_t}{d_s}\cdot \epi_t(s)$. Therefore, we have: 
\begin{align*}
\epi(t)=\frac{1}{n}\cdot \sum_{s\in V}\sum_{\ell=0}^{L} \frac{d_t}{d_s}\cdot \alpha \cdot \er^{(\ell)}_t(s). 
\end{align*}
By applying the linearity of expectation, we can derive: 
\begin{align*}
\E\left[\epi(t)\right]=\frac{1}{n}\cdot \hspace{-1mm}\sum_{s\in V}\sum_{\ell=0}^{L} \frac{d_t}{d_s}\cdot \alpha \cdot \E\left[\er^{(\ell)}_t(s)\right]=\frac{1}{n}\cdot \hspace{-1mm}\sum_{s\in V}\sum_{\ell=0}^{L} \frac{d_t}{d_s}\cdot \vpi^{(\ell)}_t(s), 
\end{align*}
where we also employ the expected value of $\er^{(\ell)}_t(s)$ given by Lemma~\ref{lem:unbiasedness_er}. We note that by Equation~\eqref{eqn:undirectedPPR}, $\frac{d_t}{d_s}\cdot \vpi^{(\ell)}_t(s)=\vpi^{(\ell)}_s(t)$. Thus,  
\begin{align*}
\E\left[\epi(t)\right]=\frac{1}{n}\cdot \sum_{s\in V}\sum_{\ell=0}^{L} \vpi^{(\ell)}_s(t)=\bpi(t), 
\end{align*}
and the lemma follows. 
\end{proof}


%\begin{theorem}[Unbiasedness]\label{thm:unbiasedness}
%Algorithm~\ref{alg:VBES} returns an unbiased estimator $\epi(t)$ for the PageRank of node $t$ that $\E[\epi(t)]=\vpi(t)$. 
%\end{theorem}
Up to now, we have proved that $\epi(t)$ is an unbiased estimator of the truncated PageRank $\vpi(t)$. Based on Lemma~\ref{lem:trunc_pagerank_approx}, next, we aim to analyze the variance of $\epi(t)$, and utilize the Chebyshev Inequality~\cite{mitzenmacher2017probability} to bound the failure probability of $\left|\epi(t)-\bpi(t)\right|\le \frac{\rela}{2}\cdot \vpi(t)$. 

\begin{fact}[Chebyshev's Inequality~\cite{mitzenmacher2017probability}]\label{fact:chebyshev}
Let $X$ denote a random variable. For any real number $\e>0$, $\Pr\left\{X-\E[X]\ge \e\right\}\le \frac{\Var[X]}{\e^2}$. 
\end{fact}

\subsection{Variance Analysis}\label{subsec:variance}
We claim that the variance of $\epi(t)$ can be bounded by $\frac{L\theta d_t}{n}\cdot \vpi(t)$, which is formally demonstrated in Theorem~\ref{thm:variance}. 

\begin{theorem}[Variance]\label{thm:variance}
The variance of the estimator $\epi(t)$ returned by Algorithm~\ref{alg:VBES} can be bounded as $\Var[\epi(t)]\le \frac{L \theta d_t }{n}\cdot \vpi(t)$. 
\end{theorem}

To prove Theorem~\ref{thm:variance}, we need several technical lemmas as shown below. Specifically, in Lemma~\ref{lem:conditional_variance}, we first bound the conditional variance of $\er^{(\ell+1)}(v)$ with the obtained residue vector $\er^{(\ell)}$. 

\begin{lemma}\label{lem:conditional_variance} 
For each node $v\in V$, the variance of $\er^{(\ell)}(v)$ obtained by Algorithm~\ref{alg:VBES} in the $(\ell+1)$-th iteration can be bounded as
\begin{align*}
\Var\left[\er^{(\ell+1)}(v)~\big|~ \er^{(\ell)}\right]\le \sum_{u\in N(v)}\th \cdot \frac{(1-\alpha)\cdot \er^{(\ell)}_t(u)}{d_u}
\end{align*}
conditioned on the residue vector $\er^{(\ell)}$ derived in the $\ell$-th iteration. 
\end{lemma}

\begin{proof}
Recall that in the proof of Lemma~\ref{lem:unbiasedness_er}, we use $\incre^{(\ell+1)}(u,v)$ to denote the probability mass transferred from node $u$ to node $v$ in the $(\ell+1)$-th iteration of Algorithm~\ref{alg:VBES}. %and we have $\er^{(\ell+1)}(v)=\sum_{u\in N(v)}\incre^{(\ell+1)}(u,v)$. Thus, we bound the variance of 
For the deterministic case when $\frac{(1-\alpha)}{d_u}\cdot \er^{(\ell)}_t(u)\ge \th$, $\incre^{(\ell+1)}(u,v)$ is deterministically set as $\frac{(1-\alpha)}{d_u}\cdot \er^{(\ell)}_t(u)$ with no variance. For the randomized case when  $\frac{(1-\alpha)}{d_u}\cdot \er^{(\ell)}_t(u)<\th$, we set $\incre^{(\ell+1)}(u,v)$ as $\th$ with probability $\frac{(1-\alpha)}{d_u\cdot \th}\cdot \er^{(\ell)}_t(u)$, or as $0$ with probability $1-\frac{(1-\alpha)}{d_u\cdot \th}\cdot \er^{(\ell)}_t(u)$. Therefore, in the randomized case, the variance of $\incre^{(\ell+1)}(u,v)$ conditioned on the residue vector $\er^{(\ell)}_t$ can be bounded as: 
\begin{equation*}
\begin{aligned}
&\Var\left[\left. \incre^{(\ell+1)}(u,v)~\right|~\er^{(\ell)}_t \right]\le \E\left[\left. \left(\incre^{(\ell+1)}(u,v)\right)^2~\right|~\er^{(\ell)}_t \right]\\
&= \th^2 \cdot \frac{(1-\alpha)}{d_u\cdot \th}\cdot \er^{(\ell)}_t(u)=\th\cdot \frac{(1-\alpha)}{d_u}\cdot \er^{(\ell)}_t(u). 
\end{aligned}
\end{equation*}
Since $\er^{(\ell+1)}(v)=\sum_{u\in N(v)}\incre^{(\ell+1)}(u,v)$, we can further derive: 
\begin{align*}
\Var\left[\left. \er^{(\ell+1)}_t(v)~\right|~\er^{(\ell)}_t \right]=\Var\left[\left. \sum_{u\in N(v)}\incre^{(\ell+1)}(u,v)~\right|~\er^{(\ell)}_t \right]. 
\end{align*}
Notably, for each $u\in N(v)$, $\incre^{(\ell+1)}(u,v)$ is independent with each other due to the independence of the binomial sampling outcomes. Thus, we can further derive: 
\begin{equation*}
\begin{aligned}
\Var\left[\hspace{-0.5mm}\left. \er^{(\ell+1)}_t\hspace{-0.5mm}(v)\right|\er^{(\ell)}_t \hspace{-0.5mm}\right]\hspace{-1mm}=\hspace{-3mm}\sum_{u\in N(v)}\hspace{-3mm}\Var\hspace{-0.5mm}\left[\hspace{-0.5mm}\left. \incre^{(\ell+1)}\hspace{-0.5mm}(u,v)\right|\er^{(\ell)}_t \hspace{-0.5mm}\right]\hspace{-1mm}\le \hspace{-3mm}\sum_{u\in N(v)}\hspace{-3.5mm}\frac{\th \hspace{-0.5mm}\cdot \hspace{-0.5mm}(1\hspace{-0.5mm}-\hspace{-0.5mm}\alpha)}{d_u}\hspace{-0.5mm}\cdot \hspace{-0.5mm}\er^{(\ell)}_t\hspace{-0.5mm}(u), 
\end{aligned}    
\end{equation*}
which follows the lemma. 
\end{proof}

In the second step, we prove: 
\begin{lemma}\label{lem:var_recur}
The variance of the estimator $\epi(t)$ obtained by Algorithm~\ref{alg:VBES} can be computed as: 
\begin{equation*}
\begin{aligned}
&\Var\left[\epi(t)\right]=\frac{\alpha^2}{n^2}\cdot \Var\left[\sum_{\ell=0}^L \sum_{s\in V}\frac{d_t}{d_s}\cdot \er^{(\ell)}_t(s)\right]\\
&=\hspace{-0.5mm}\frac{\alpha^2}{n^2}\hspace{-0.5mm}\cdot \sum_{\ell=0}^{L-2}\hspace{-0.5mm}\E\left[\Var\hspace{-0.5mm}\left[\left.\sum_{v\in V}\left(\sum_{s\in V}\frac{d_t}{d_s}\cdot \hspace{-1mm}\sum_{i=0}^{L-\ell-1}\hspace{-0.5mm}\frac{\vpi^{(i)}_v\hspace{-0.5mm}(s)}{\alpha}\right)\cdot \hspace{-0.5mm}\er^{(\ell+1)}_t(v)~\right|~\er^{(\ell)}_t\right]\right]. 
\end{aligned}    
\end{equation*}
\end{lemma}
To prove Lemma~\ref{lem:var_recur}, recall that $\epi(t)=\frac{1}{n}\sum_{s\in V}\frac{d_t}{d_s}\cdot \epi_t(s)$, and $\epi_t(s)=\sum_{\ell=0}^L \alpha \er^{(\ell)}_t(s)$ according to Algorithm~\ref{alg:VBES}. Thus, the variance of $\epi(t)$ derived by Algorithm~\ref{alg:VBES} can be computed as: 
\begin{align*}
\Var\hspace{-0.5mm}\left[\epi(t)\right]\hspace{-0.5mm}=\hspace{-0.5mm}\Var\left[\hspace{-0.5mm}\frac{1}{n}\hspace{-0.5mm}\cdot \hspace{-1mm}\sum_{s\in V}\hspace{-0.5mm}\frac{d_t}{d_s}\hspace{-0.5mm}\cdot \hspace{-1mm}\sum_{\ell=0}^{L}\hspace{-0.5mm}\alpha \hspace{-0.5mm}\cdot \hspace{-0.5mm}\er_t^{(\ell)}\hspace{-0.5mm}(s)\hspace{-0.5mm}\right]\hspace{-1mm}=\hspace{-0.5mm}\frac{\alpha^2}{n^2}\hspace{-0.5mm}\cdot \hspace{-0.5mm}\Var\left[\sum_{s\in V}\hspace{-1mm}\frac{d_t}{d_s}\hspace{-1mm}\cdot \hspace{-1mm}\sum_{\ell=0}^{L}\hspace{-0.5mm}\er_t^{(\ell)}\hspace{-0.5mm}(s)\hspace{-0.5mm}\right], 
\end{align*}
following the first equality in Lemma~\ref{lem:var_recur}. For the second equality in Lemma~\ref{lem:var_recur},  the detailed proof is rather technical, and we defer it to the Technical Report~\cite{TechnicalReport} for readability. Intuitively, we can prove it by iteratively applying the law of total variance as shown in Fact~\ref{fact:totalvar}. 

\begin{fact}[Law of Total Variance~\cite{weiss2005TotalVarianceLaw}]\label{fact:totalvar}
For two random variables $X$ and $Y$, the law of total variance states: 
\begin{align*}
\Var\left[Y\right]=\E\left[\Var \left[Y\mid X\right]\right]+\Var\left[\E\left[Y\mid X\right]\right]
\end{align*}
holds if the two variables $X$ and $Y$ are on the same probability space and the variance of $Y$ is finite. 
\end{fact}

Furthermore, we apply the results in Lemma~\ref{lem:conditional_variance} to the expression given by Lemma~\ref{lem:var_recur}, which follows Lemma~\ref{lem:var_partial}. 

\begin{lemma}\label{lem:var_partial}
For all $\ell\in [0, L]$, the residue vectors $\er^{(\ell)}$ obtained by Algorithm~\ref{alg:VBES} in the $\ell$-th iterations satisfy: 
\begin{equation*}
\begin{aligned}
\sum_{\ell=0}^{L-2}\hspace{-0.5mm}\E\hspace{-0.5mm}\left[\hspace{-0.5mm}\Var\hspace{-0.5mm}\left[\hspace{-0.5mm}\left.\sum_{v\in V}\hspace{-0.5mm}\left(\sum_{s\in V}\hspace{-0.8mm}\frac{d_t}{d_s}\hspace{-0.5mm}\cdot \hspace{-0.5mm}\hspace{-0.5mm}\sum_{i=0}^{L-\ell-1}\hspace{-1.5mm}\frac{\vpi^{(i)}_v\hspace{-0.5mm}(s)}{\alpha}\hspace{-0.5mm}\right)\hspace{-0.5mm}\cdot \hspace{-0.5mm}\er^{(\ell+1)}_t\hspace{-0.5mm}(v)~\right|\er^{(\ell)}_t\hspace{-0.5mm}\right]\right]\hspace{-1mm}\le \hspace{-0.5mm}\frac{ L\th d_t \hspace{-0.5mm}\cdot \hspace{-0.5mm} n\vpi(t)}{\alpha^2}. 
\end{aligned}    
\end{equation*}
\end{lemma}

\begin{proof} 
Recall that in the $(\ell+1)$-th iteration of Algorithm~\ref{alg:VBES}, we set $\er^{(\ell+1)}(v)=\sum_{u\in N(v)}\incre^{(\ell+1)}(u,v)$. And the value of $\incre^{(\ell+1)}(u,v)$ is independent from other $\incre^{(\ell+1)}(x,y)$ for $\forall (x, y) \in E$ based on the derived residue vectors $\er^{(j)}_t$ for $j\in \{0, 1, \ldots, \ell\}$. Therefore, for each $v\in V$, $\er^{(\ell+1)}_t(v)$ is independent with each other, which follows: 
\begin{equation}\label{eqn:exp_sum}
\begin{aligned}
&\sum_{\ell=0}^{L-2}\E\left[\Var\left[\left.\sum_{v\in V}\left(\sum_{s\in V}\frac{d_t}{d_s}\cdot \hspace{-1mm}\sum_{i=0}^{L-\ell-1}\frac{\vpi^{(i)}_v(s)}{\alpha}\right)\cdot \er^{(\ell+1)}_t(v)~\right|\er^{(\ell)}_t\right]\right]\\
&=\sum_{\ell=0}^{L-2}\E\left[\sum_{v\in V}\Var\left[\left.\left(\sum_{s\in V}\frac{d_t}{d_s}\cdot \hspace{-1mm}\sum_{i=0}^{L-\ell-1}\frac{\vpi^{(i)}_v(s)}{\alpha}\right)\cdot \er^{(\ell+1)}_t(v)~\right|\er^{(\ell)}_t\right]\right]. 
\end{aligned}    
\end{equation}
Note that $\sum_{s\in V}\frac{d_t}{d_s}\cdot \hspace{-1mm}\sum_{i=0}^{L-\ell-1}\frac{\vpi^{(i)}_v(s)}{\alpha}$ is a parameter, instead of a random variable, which can be bounded as: 
\begin{align*}
\sum_{s\in V}\frac{d_t}{d_s}\cdot \hspace{-2mm}\sum_{i=0}^{L-\ell-1}\hspace{-1mm}\frac{\vpi^{(i)}_v(s)}{\alpha}\le \frac{d_t}{\alpha}\cdot \hspace{-1mm}\sum_{s\in V}\sum_{i=0}^{L-\ell-1}\hspace{-1mm}\vpi^{(i)}_v(s) \le \frac{d_t}{\alpha}\cdot \hspace{-1mm} \sum_{s\in V}\vpi_v(s)=\frac{d_t}{\alpha}. 
\end{align*}
Therefore, by plugging the upper bound of $\sum_{s\in V}\frac{d_t}{d_s}\cdot \sum_{i=0}^{L-\ell-1}\frac{\vpi^{(i)}_v(s)}{\alpha}$ into Equation~\eqref{eqn:exp_sum}, we can further derive: 
\begin{equation*}
\begin{aligned}
&\sum_{\ell=0}^{L-2}\E\left[\sum_{v\in V}\Var\left[\left.\left(\sum_{s\in V}\frac{d_t}{d_s}\cdot \hspace{-1mm}\sum_{i=0}^{L-\ell-1}\frac{\vpi^{(i)}_v(s)}{\alpha}\right)\cdot \er^{(\ell+1)}_t(v)~\right|\er^{(\ell)}_t\right]\right]\\
&\le \hspace{-1mm}\frac{d_t}{\alpha}\cdot \hspace{-1mm}\sum_{\ell=0}^{L-2}\E\left[\sum_{v\in V}\left(\sum_{s\in V}\frac{d_t}{d_s}\cdot \hspace{-1mm}\sum_{i=0}^{L-\ell-1}\frac{\vpi^{(i)}_v(s)}{\alpha}\right)\cdot \Var\left[\left. \er^{(\ell+1)}_t(v)~\right|\er^{(\ell)}_t\right]\right]. 
\end{aligned}    
\end{equation*}
By Lemma~\ref{lem:conditional_variance}, we have: 
%\begin{align*}
$\Var\left[\left. \er^{(\ell+1)}_t(v)~\right|\er^{(\ell)}_t\right]\hspace{-1mm}\le \hspace{-0.5mm}\sum_{u\in N(v)}\hspace{-0.5mm}\frac{\th \cdot (1-\alpha)\cdot \er^{(\ell)}_t(u)}{d_u}$, 
%\end{align*}
and thus, by Lemma~\ref{lem:unbiasedness_er} and Equation~\eqref{eqn:PPR_recur}, it follows: 
\begin{equation*}
\begin{aligned}
&\E\left[\Var\left[\left. \er^{(\ell+1)}_t(v)~\right|\er^{(\ell)}_t\right]\right]\le \sum_{u\in N(v)}\frac{\th \cdot (1-\alpha)}{d_u}\cdot \E\left[\er^{(\ell)}_t(u)\right]\\
&=\sum_{u\in N(v)} \frac{\th \cdot (1-\alpha)}{\alpha \cdot d_u}\cdot \vpi^{(\ell)}_t(u)=\frac{\th}{\alpha}\cdot \vpi^{(\ell+1)}_t(v). 
\end{aligned}    
\end{equation*}
Plugging the above inequality into Equation~\eqref{eqn:exp_sum}, we have: 
\begin{equation*}
\begin{aligned}
&\sum_{\ell=0}^{L-2}\E\left[\sum_{v\in V}\Var\left[\left.\left(\sum_{s\in V}\frac{d_t}{d_s}\cdot \hspace{-1mm}\sum_{i=0}^{L-\ell-1}\frac{\vpi^{(i)}_v(s)}{\alpha}\right)\cdot \er^{(\ell+1)}_t(v)~\right|\er^{(\ell)}_t\right]\right]\\
& \le \frac{d_t \cdot \th}{\alpha^2}\cdot \sum_{\ell=0}^{L-2} \sum_{s\in V}\frac{d_t}{d_s}\cdot \sum_{i=0}^{L-\ell-1}\sum_{v\in V} \frac{\vpi^{(i)}_v(s)}{\alpha} \cdot \vpi^{(\ell+1)}_t(v). 
%=\frac{d_t\cdot \th}{\alpha^2}\cdot \sum_{\ell=0}^{L-2} \sum_{s\in V}\frac{d_t}{d_s}\cdot \hspace{-2mm}\sum_{i=0}^{L-\ell-1}\vpi^{(\ell+i+1)}_t(s). 
\end{aligned}    
\end{equation*}
We note $\sum_{v\in V}\frac{1}{\alpha}\cdot \vpi^{(i)}_v(s)\cdot \vpi^{(\ell+1)}_t(v)=\vpi^{(\ell+1+i)}_t(s)$ and 
\begin{align*}
\sum_{s\in V}\frac{d_t}{d_s}\cdot \sum_{i=0}^{L-\ell-1}\vpi^{(\ell+1+i)}_t(s)\le \sum_{s\in V}\frac{d_t}{d_s}\cdot \vpi_t(s)=\sum_{s\in V} \vpi_s(t)=n\vpi(t). 
\end{align*}
As a consequence, we can further derive: 
\begin{equation*}
\begin{aligned}
&\sum_{\ell=0}^{L-2}\E\left[\Var\left[\left.\sum_{v\in V}\left(\sum_{s\in V}\frac{d_t}{d_s}\cdot \hspace{-1mm}\sum_{i=0}^{L-\ell-1}\frac{\vpi^{(i)}_v(s)}{\alpha}\right)\cdot \er^{(\ell+1)}_t(v)~\right|\er^{(\ell)}_t\right]\right]\\
&\le \frac{d_t \cdot \th}{\alpha^2} \cdot \sum_{\ell=0}^{L-2} n\pi(t) \le \frac{1}{\alpha^2} \cdot L \th d_t \cdot n \vpi(t), 
\end{aligned}   
\end{equation*}
following the lemma. 
\end{proof}

Finally, putting Lemma~\ref{lem:var_recur} and ~\ref{lem:var_partial} together, we can conclude that  
%\begin{align*}
$\Var\left[\epi(t)\right]\le \frac{L\cdot \th \cdot d_t}{n^2}\cdot n\epi(t)$, 
%\end{align*}
following Theorem~\ref{thm:variance}. 


\subsection{Time Cost}\label{subsec:totalcost}
In the following, we analyze the expected time cost of the \setpush algorithm. Moreover, Theorem~\ref{thm:finalcost_analysis} provides the theoretical guarantees of the \setpush algorithm for achieving a $(\rela, \pf)$-approximation of the single-node PageRank. 

\begin{lemma}\label{lem:cost_theta}
The expected time cost of Algorithm~\ref{alg:VBES} can be bounded by ${\rev \frac{1}{\alpha \theta}=}~O\left(\frac{1}{\th}\right)$. 
\end{lemma} 

\begin{proof}
Let $Cost^{(\ell+1)}(u,v)$ denote the time cost for pushing the probability mass from node $u$ to node $v$ in the $(\ell+1)$-th iteration of Algorithm~\ref{alg:VBES}. Thus, $Cost^{(\ell+1)}(u,v)=1$ deterministically in the deterministic case when $\frac{(1-\alpha)}{d_u}\cdot \er^{(\ell)}_t(u)\ge \th$. On the other hand, for the randomized case, $Cost^{(\ell+1)}(u,v)=1$ (i.e., pushing probability mass from node $u$ to $v$) with probability $\frac{(1-\alpha)}{d_u\cdot \th}\cdot \er^{(\ell)}_t(u)$, and $Cost^{(\ell+1)}(u,v)=0$ with probability $1-\frac{(1-\alpha)}{d_u\cdot \th}\cdot \er^{(\ell)}_t(u)$. Thus, for the randomized case, 
\begin{align*}
\E\left[Cost^{(\ell+1)}(u,v)~\big|~ \er^{(\ell)}_t\right]=1\cdot \frac{(1-\alpha)}{d_u\cdot \th}\cdot \er^{(\ell)}_t(u). 
\end{align*}
Furthermore, we use $Cost^{(\ell+1)}$ to denote the time cost of the $(\ell+1)$-th iteration in Algorithm~\ref{alg:VBES}. Since $Cost^{(\ell+1)}\hspace{-0.5mm}=\hspace{-0.5mm}\sum_{(u,v)\in E} Cost^{(\ell+1)}(u,v)$, we can derive: 
\begin{equation*}
\begin{aligned}
\E\hspace{-0.5mm}\left[Cost^{(\ell+1)}~\big|~ \er^{(\ell)}_t\hspace{-0.5mm}\right]\hspace{-0.5mm}=\hspace{-3mm}\sum_{(u,v)\in E}\hspace{-2.5mm}\E\left[Cost^{(\ell+1)}(u,v)~\big|~ \er^{(\ell)}_t\hspace{-0.5mm}\right]\hspace{-0.5mm}=\hspace{-3mm}\sum_{(u,v)\in E}\hspace{-2mm}\frac{(1\hspace{-0.5mm}-\hspace{-0.5mm}\alpha)}{d_u \hspace{-0.5mm}\cdot \hspace{-0.5mm}\th}\hspace{-0.5mm}\cdot \er^{(\ell)}_t\hspace{-0.5mm}(u). 
%1\cdot \frac{(1-\alpha)}{d_u\cdot \th}\cdot \er^{(\ell)}_t(u). 
\end{aligned}    
\end{equation*}
It follows: 
\begin{equation*}
\begin{aligned}
&\E\left[Cost^{(\ell+1)}\right]=\E\left[\E\left[Cost^{(\ell+1)}~\big|~ \er^{(\ell)}_t\hspace{-0.5mm}\right]\right]=\hspace{-2mm}\sum_{(u,v)\in E}\hspace{-1mm}\frac{(1\hspace{-0.5mm}-\hspace{-0.5mm}\alpha)}{d_u \hspace{-0.5mm}\cdot \hspace{-0.5mm}\th}\hspace{-0.5mm}\cdot \E\left[\er^{(\ell)}_t\hspace{-0.5mm}(u)\right]\\
&=\frac{1}{\alpha\th}\cdot \sum_{v\in V}\sum_{u\in N(v)}\hspace{-2mm}\frac{(1\hspace{-0.5mm}-\hspace{-0.5mm}\alpha)}{d_u}\hspace{-0.5mm}\cdot \vpi^{(\ell)}_t\hspace{-0.5mm}(u)=\frac{1}{\alpha\th}\cdot \sum_{v\in V}\vpi^{(\ell+1)}_t(v),  
\end{aligned}
\end{equation*}
where we apply Lemma~\ref{lem:unbiasedness_er} in the third equality, and Equation~\eqref{eqn:PPR_recur} in the last equality. We further use $Cost=\sum_{\ell=0}^{L-1}Cost^{(\ell+1)}$ to denote the total time cost of Algorithm~\ref{alg:VBES}. Thus, we have: 
\begin{align*}
\E\left[Cost\right]=\hspace{-0.5mm}\sum_{\ell=0}^{L-1}\E\left[Cost^{(\ell+1)}\right]\hspace{-0.5mm}=\hspace{-0.5mm}\frac{1}{\alpha\th}\cdot \hspace{-1mm}\sum_{v\in V}\sum_{\ell=0}^{L-1}\vpi^{(\ell+1)}_t(v)\hspace{-0.5mm}\le \hspace{-0.5mm}\frac{1}{\alpha\th}=O\left(\frac{1}{\th}\right),  
\end{align*}
by applying the fact that $\sum_{\ell=0}^{L-1}\vpi^{(\ell+1)}_t(v)\le \vpi_t(v)$, and $\sum_{v\in V}\vpi^{(\ell+1)}_t(v)$. Therefore, the lemma follows. 
\end{proof}

At the end, we employ the bound of variance $\Var\left[\epi(t)\right]$ derived in Theorem~\ref{thm:variance} to the Chebyshev's Inequality given in Fact~\ref{fact:chebyshev}, and thus obtain the required setting of threshold $\theta$. As shown in Theorem~\ref{thm:finalcost_analysis}, by setting $\theta$ roughly proportional to the value of $\max\left\{\frac{1}{d_t}, \frac{1}{\sqrt{m}}\right\}$, the \setpush algorithm achieves a $(\rela, \pf)$-approximation of $\vpi(t)$. Plugging the setting of $\theta$ to the results given by Lemma~\ref{lem:cost_theta}, the expected time cost can be further bounded by $\tilde{O}\left(\min\left\{d_t,\sqrt{m}\right\}\right)$.  


\begin{figure*}[t]
\begin{minipage}[t]{1\textwidth}
\centering
\vspace{+2mm}
%    \begin{footnotesize}
\begin{tabular}{cccc}
\hspace{-4mm} \includegraphics[width=45mm]{./Figs/query time_YT_01.pdf} &
\hspace{-3mm} \includegraphics[width=45mm]{./Figs/query time_IC_01.pdf} &
\hspace{-3mm} \includegraphics[width=45mm]{./Figs/query time_OL_01.pdf} &
\hspace{-3mm} \includegraphics[width=45mm]{./Figs/query time_FR_01.pdf} \\
\end{tabular}
\vspace{-4mm}
\caption{Query time (seconds) of each algorithm with uniformly selected query node and $\rela=0.1$}
\label{fig:query_uniform_0.1}
\vspace{+2mm}
\end{minipage}

\begin{minipage}[t]{1\textwidth}
\centering
%\vspace{-5mm}
%    \begin{footnotesize}
\begin{tabular}{cccc}
\hspace{-4mm} \includegraphics[width=45mm]{./Figs/query time_YT_05.pdf} &
\hspace{-3mm} \includegraphics[width=45mm]{./Figs/query time_IC_05.pdf} &
\hspace{-3mm} \includegraphics[width=45mm]{./Figs/query time_OL_05.pdf} &
\hspace{-3mm} \includegraphics[width=45mm]{./Figs/query time_FR_05.pdf} \\
\end{tabular}
\vspace{-4mm}
\caption{Query time (seconds) of each algorithm with uniformly selected query node and $\rela=0.5$}
\label{fig:query_uniform_0.5}
\vspace{+2mm}
\end{minipage}
\end{figure*}



\begin{theorem}\label{thm:finalcost_analysis}
By setting $\theta=\max\left\{\frac{\alpha c^2}{12L\cdot d_t},\frac{\alpha c^2}{12L}\hspace{-0.5mm}\cdot \hspace{-0.5mm}\sqrt{\frac{2(1-\alpha)}{m}}\right\}$, Algorithm~\ref{alg:VBES} returns an estimator $\epi(t)$ of $\vpi(t)$, such that $|\vpi(t)-\epi(t)|\le c\cdot \vpi(t)$ holds with constant probability. The expected time cost of Algorithm~\ref{alg:VBES} is bounded by 
\begin{align*}
{\rev 
\frac{12 \cdot \left(\log_{1-\alpha}\frac{c\alpha}{2n}\right)}{\alpha^2 c^2}\cdot \min \left\{d_t, \sqrt{\frac{m}{2(1-\alpha)}}\right\}
}
~=\tilde{O}\left(\min\left\{d_t,\sqrt{m}\right\}\right). 
\end{align*} 
%\begin{enumerate}
%\item If we set $\theta=\tilde{O}\left(\frac{1}{\sqrt{m}}\right)$, then the expected time cost of Algorithm~\ref{alg:VBES} is bounded by $\tilde{O}\left(\sqrt{m}\right)$.  
%\item If we set $\theta=\tilde{O}\left(\frac{1}{\sqrt{m}}\right)$, then the expected time cost of Algorithm~\ref{alg:VBES} is bounded by $\tilde{O}\left(\sqrt{m}\right)$. 
%\end{enumerate}
%\vspace{-1mm}
\end{theorem}

\begin{proof} %To prove Theorem~\ref{thm:finalcost_analysis}, we utilize the Chebyshev's Inequality as shown below to bound the value of $\th$. 
Recall that the variance of $\epi(t)$ obtained by Algorithm~\ref{alg:VBES} is bounded by $\frac{L\cdot \th \cdot d_t}{n^2}\cdot n\epi(t)$ given in Theorem~\ref{thm:variance}. By the Chebyshev's Inequality, we have: 
\begin{align*}
\Pr\left\{\epi(t)-\bpi(t)\ge \frac{c}{2} \cdot \vpi(t)\right\} \le \frac{4 \cdot \Var\left[\epi(t)\right]}{c^2 \cdot \left(\vpi(t)\right)^2}\le \frac{4L\th d_t}{c^2 \cdot n\vpi(t)}. 
\end{align*}
Thus, by setting $\th= \frac{c^2 \cdot n\vpi(t)}{12Ld_t}$, $\epi(t)-\bpi(t)\le \frac{c}{2} \cdot \vpi(t)$ holds with probability at least $\frac{1}{3}$. In particular, we note $\frac{c^2 \cdot n\vpi(t)}{12Ld_t}\ge \frac{\alpha c^2}{12Ld_t}$ based on the fact that $\vpi(t)\ge \frac{\alpha}{n}$ as illustrated in Equation~\eqref{eqn:ite_pagerank}. If we set $\theta=\frac{\alpha c^2}{12Ld_t}$, then according to Lemma~\ref{lem:cost_theta}, the expected time cost of Algorithm~\ref{alg:VBES} can be bounded by %$O\left(\frac{1}{\th}\right)=O\left(\frac{12Ld_t}{\alpha c^2}\right)=\tilde{O}\left(d_t\right)$ with $L=\log_{1-\alpha}{\frac{c\alpha}{2n}}$ and the constants $\alpha$ and $c$. 
{\rev 
$\frac{1}{\alpha \theta}=\frac{12L d_t}{\alpha^2 c^2}=\tilde{O}\left(d_t\right)$ because $L=\log_{1-\alpha}{\frac{c\alpha}{2n}}=\tilde{O}(1)$ (see Section~\ref{subsec:trunc_pagerank} for the details of setting $L$) and $\alpha, c$ are constants. 
}
Moreover, as we shall prove below, $\frac{n \vpi(t)}{d_t}\hspace{-0.5mm}\ge \hspace{-0.5mm}\alpha  \hspace{-0.5mm} \cdot  \hspace{-0.5mm}\sqrt{\frac{2(1-\alpha)}{m}}$ holds for any $t\in V$. Thus, by setting $\th \hspace{-0.5mm}= \hspace{-0.5mm}\frac{\alpha c^2}{12L}\hspace{-0.5mm}\cdot \hspace{-0.5mm}\sqrt{\frac{2(1-\alpha)}{m}}$, the expected time cost of Algorithm~\ref{alg:VBES} is bounded by 
%$O\left(\hspace{-0.5mm}\frac{1}{\th}\hspace{-0.5mm}\right)\hspace{-0.5mm}=\hspace{-0.5mm}O\left(\frac{12L}{\alpha c^2}\hspace{-0.5mm}\cdot \hspace{-1mm}\sqrt{\frac{m}{2(1-\alpha)}}\right)=\tilde{O}\left(\hspace{-0.5mm}\sqrt{m}\right)$. 
{\rev 
$\frac{1}{\alpha \theta}=\frac{12L}{\alpha^2 c^2}\hspace{-0.5mm}\cdot \hspace{-1mm}\sqrt{\frac{m}{2(1-\alpha)}}=\tilde{O}(\sqrt{m})$, where, analogously, $L=\log_{1-\alpha}{\frac{c\alpha}{2n}}=\tilde{O}(1)$ and $\alpha, c$ are constants. 
}

Now we present the proof of $\frac{n \vpi(t)}{d_t}\hspace{-0.5mm}\ge \hspace{-0.5mm}\alpha \cdot \sqrt{\frac{2(1-\alpha)}{m}}$. By Equation~\eqref{eqn:ite_pagerank}, we have: 
\begin{equation}\label{eqn:sqrtm}
\begin{aligned}
\vpi(t)\ge (1-\alpha)\hspace{-2mm}\sum_{u\in N(t)}\hspace{-1mm}\frac{\vpi(u)}{d_u}+\frac{\alpha}{n} \ge (1-\alpha)\hspace{-1mm}\sum_{u\in N(t)}\frac{1}{d_u}\cdot \frac{\alpha}{n}+\frac{\alpha}{n}. %=\frac{\alpha}{n} \cdot \left(\sum_{u\in N(t)}\frac{(1-\alpha)}{d_u}\right). 
\end{aligned}    
\end{equation}
We note $\sum_{u\in N(t)}\hspace{-1mm}\frac{1}{d_u}\hspace{-0.5mm}\ge \hspace{-0.5mm}\frac{d_t^2}{2m}$ since
%\begin{align*}
$\left(\sum_{u\in N(t)}\frac{1}{d_u}\right)\cdot \left(\sum_{u\in N(t)}d_u\right)\ge \left(\sum_{u\in N(t)}1\right)^2=d_t^2$ 
%\end{align*}
holds by the Cauchy-Schwarz Inequality~\cite{steele2004cauchy}. Plugging into Inequality~\eqref{eqn:sqrtm}, we can further derive: 
\begin{align*}
\vpi(t)\hspace{-0.5mm}\ge \hspace{-0.5mm}\frac{\alpha}{n}\hspace{-0.5mm}\cdot \hspace{-0.5mm}\left(\frac{(1-\alpha)d_t^2}{2m}\hspace{-0.5mm}+\hspace{-0.5mm}1\right)\hspace{-0.5mm}=\hspace{-0.5mm}\frac{\alpha d_t}{n}\hspace{-0.5mm}\cdot\hspace{-0.5mm} \left(\frac{(1-\alpha)d_t\hspace{-0.5mm}+\hspace{-0.5mm}\frac{2m}{d_t}}{2m}\right)\hspace{-0.5mm}\ge \hspace{-0.5mm}\frac{\alpha d_t}{n}\hspace{-0.5mm}\cdot \hspace{-0.5mm}\sqrt{\frac{2(1\hspace{-0.5mm}-\hspace{-0.5mm}\alpha)}{m}}, 
\end{align*}
where we apply the fact that $(1-\alpha)d_t+\frac{2m}{d_t} \ge 2\cdot \sqrt{(1-\alpha)2m}$ by the AM-GM Inequality. Consequently, $\frac{n \vpi(t)}{d_t}\hspace{-0.5mm}\ge \hspace{-0.5mm}\alpha \cdot \sqrt{\frac{2(1-\alpha)}{m}}$ holds for each $t\in V$, and the theorem follows. 
\end{proof}


\begin{comment}
\begin{proof} %To prove Theorem~\ref{thm:finalcost_analysis}, we utilize the Chebyshev's Inequality as shown below to bound the value of $\th$. 
Recall that the variance of $\epi(t)$ obtained by Algorithm~\ref{alg:VBES} is bounded by $\frac{L\cdot \th \cdot d_t}{n^2}\cdot n\epi(t)$ given in Theorem~\ref{thm:variance}. By the Chebyshev's Inequality, we have: 
\begin{align*}
\Pr\left\{\epi(t)-\bpi(t)\ge \frac{c}{2} \cdot \vpi(t)\right\} \le \frac{4 \cdot \Var\left[\epi(t)\right]}{c^2 \cdot \left(\vpi(t)\right)^2}\le \frac{4L\th d_t}{c^2 \cdot n\vpi(t)}. 
\end{align*}
Thus, by setting $\th= \frac{c^2 \cdot n\vpi(t)}{12Ld_t}$, $\epi(t)-\bpi(t)\le \frac{c}{2} \cdot \vpi(t)$ holds with probability at least $\frac{1}{3}$. In particular, we note $\frac{c^2 \cdot n\vpi(t)}{12Ld_t}\ge \frac{\alpha c^2}{12Ld_t}$ based on the fact that $\vpi(t)\ge \frac{\alpha}{n}$ as illustrated in Equation~\eqref{eqn:ite_pagerank}. If we set $\theta=\frac{\alpha c^2}{12Ld_t}$, then the expected time cost of Algorithm~\ref{alg:VBES} can be bounded by $O\left(\frac{1}{\th}\right)=O\left(\frac{12Ld_t}{\alpha c^2}\right)=\tilde{O}\left(d_t\right)$ with $L=\log_{1-\alpha}{\frac{c\alpha}{2n}}$ and the constants $\alpha$ and $c$. Moreover, as we shall prove below, $\frac{n \vpi(t)}{d_t}\hspace{-0.5mm}\ge \hspace{-0.5mm}\alpha  \hspace{-0.5mm} \cdot  \hspace{-0.5mm}\sqrt{\frac{2(1-\alpha)}{m}}$ holds for any $t\in V$. Thus, by setting $\th \hspace{-0.5mm}= \hspace{-0.5mm}\frac{\alpha c^2}{12L}\hspace{-0.5mm}\cdot \hspace{-0.5mm}\sqrt{\frac{2(1-\alpha)}{m}}$, the expected time cost of Algorithm~\ref{alg:VBES} is bounded by $O\left(\hspace{-0.5mm}\frac{1}{\th}\hspace{-0.5mm}\right)\hspace{-0.5mm}=\hspace{-0.5mm}O\left(\frac{12L}{\alpha c^2}\hspace{-0.5mm}\cdot \hspace{-1mm}\sqrt{\frac{m}{2(1-\alpha)}}\right)=\tilde{O}\left(\hspace{-0.5mm}\sqrt{m}\right)$. Now we present the proof of $\frac{n \vpi(t)}{d_t}\hspace{-0.5mm}\ge \hspace{-0.5mm}\alpha \cdot \sqrt{\frac{2(1-\alpha)}{m}}$. By Equation~\eqref{eqn:ite_pagerank}, we have: 
\begin{equation}\label{eqn:sqrtm}
\begin{aligned}
\vpi(t)\ge (1-\alpha)\hspace{-2mm}\sum_{u\in N(t)}\hspace{-1mm}\frac{\vpi(u)}{d_u}+\frac{\alpha}{n} \ge (1-\alpha)\hspace{-1mm}\sum_{u\in N(t)}\frac{1}{d_u}\cdot \frac{\alpha}{n}+\frac{\alpha}{n}. %=\frac{\alpha}{n} \cdot \left(\sum_{u\in N(t)}\frac{(1-\alpha)}{d_u}\right). 
\end{aligned}    
\end{equation}
We note $\sum_{u\in N(t)}\hspace{-1mm}\frac{1}{d_u}\hspace{-0.5mm}\ge \hspace{-0.5mm}\frac{d_t^2}{2m}$ since
%\begin{align*}
$\left(\sum_{u\in N(t)}\frac{1}{d_u}\right)\cdot \left(\sum_{u\in N(t)}d_u\right)\ge \left(\sum_{u\in N(t)}1\right)^2=d_t^2$ 
%\end{align*}
holds by the Cauchy-Schwarz Inequality~\cite{steele2004cauchy}. Plugging into Inequality~\eqref{eqn:sqrtm}, we can further derive: 
\begin{align*}
\vpi(t)\hspace{-0.5mm}\ge \hspace{-0.5mm}\frac{\alpha}{n}\hspace{-0.5mm}\cdot \hspace{-0.5mm}\left(\frac{(1-\alpha)d_t^2}{2m}\hspace{-0.5mm}+\hspace{-0.5mm}1\right)\hspace{-0.5mm}=\hspace{-0.5mm}\frac{\alpha d_t}{n}\hspace{-0.5mm}\cdot\hspace{-0.5mm} \left(\frac{(1-\alpha)d_t\hspace{-0.5mm}+\hspace{-0.5mm}\frac{2m}{d_t}}{2m}\right)\hspace{-0.5mm}\ge \hspace{-0.5mm}\frac{\alpha d_t}{n}\hspace{-0.5mm}\cdot \hspace{-0.5mm}\sqrt{\frac{2(1\hspace{-0.5mm}-\hspace{-0.5mm}\alpha)}{m}}, 
\end{align*}
where we apply the fact that $(1-\alpha)d_t+\frac{2m}{d_t} \ge 2\cdot \sqrt{(1-\alpha)2m}$ by the AM-GM Inequality. Consequently, $\frac{n \vpi(t)}{d_t}\hspace{-0.5mm}\ge \hspace{-0.5mm}\alpha \cdot \sqrt{\frac{2(1-\alpha)}{m}}$ holds for each $t\in V$, and the theorem follows. 
\end{proof}
\end{comment}


==> applications.tex <==

\section{Applications} \label{sec:applications}

detailed description

\header{\bf Propagation in node proximity.} 
\begin{itemize}
	\item PageRank
	\item PPR
	\item HKPR
\end{itemize}
 

\header{\bf Propagation in GNN.} 
\begin{itemize}
	\item SGC
	\item GCN
	\item APPNP
	\item GDC
\end{itemize}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> optimization.tex <==
\section{Optimization} \label{sec:opt}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

==> response.tex <==
\clearpage
\setcounter{page}{1}
\setcounter{figure}{0} 
\renewcommand\thefigure{R.\arabic{figure}}
\setcounter{table}{0}
\renewcommand\thetable{R.\arabic{table}}
\setcounter{equation}{0}
\section*{author response} \label{sec:response}
%We thank the reviewers for the insightful and constructive comments. Following the suggestions, we revise our paper and the major changes are highlighted in {\hz blue}. Our responses to the major concerns of reviewers are as follows. 
We thank the reviewers for their insightful and constructive comments. Based on the reviewers' suggestions, the major changes we made in the revised paper can be summarized as three aspects: 
\begin{itemize}
\vspace{-1mm}
\item {\bf Theoretical Analyses: } (for Meta-Reviewer and Reviewer 2) 
    

    
\item {\bf Applicability Illustrations: } (for Reviewer 2)  
    

    
\item {\bf Supplementary Experiments: } (for Reviewers 1, 2 and 3) 
    

\end{itemize}

In the revised paper, the major changes were highlighted in {\rev blue}. Our responses to the major concerns of reviewers were as follows. For readability, we also presented the supplementary tables and figures in the response letter, with captions beginning with R.1. 


\subsection*{Meta-Reviewer} \label{sec:meta}
\review{\bf D1}: {\em Your results are applicable to undirected graphs. Since most of the competitors in previous research addresses directed graphs, please clarify which of the complexities (query times) in Table 1 refer only to undirected graphs and what is the best result applicable to undirected graphs. Please also comment on whether the proposed approach extends to directed graphs.} 

\header{\bf Response: } Thanks for pointing out this issue. In Table~\ref{tbl:comparison}, the complexities of LocalPush~\cite{lofgren2013personalized}, FastPPR~\cite{lofgren2014FastPPR}, BiPPR~\cite{lofgren2016BiPPR}, and our \setpush are only applicable to undirected graphs. In comparison, the complexities of the Power Method~\cite{page1999pagerank}, Monte-Carlo~\cite{fogaras2005MC}, RBS~\cite{wang2020RBS}, and \sublinear~\cite{bressan2018sublinear} hold both on directed and undirected graphs. We revised Table~\ref{tbl:comparison} by marking the complexity with a $\star$ if it is only applicable on undirected graphs. 

To our knowledge, the best complexities for single-node PageRank computations on undirected graphs are achieved by FastPPR, BiPPR and \sublinear. However, the three methods are originally proposed on directed graphs. This reflects existing methods do not make full use of the properties that PageRank scores hold on undirected graphs. This also offers us motivations to focus on the single-node PageRank computation problem on undirected graphs.  

Based on this advice, we further revised our paper in three points as shown below. 
%Furthermore, in the revised paper, we made the following changes . 

\begin{itemize}
    \item In the Abstract, we highlighted our motivations that we aim to efficiently compute single-node PageRank on undirected graphs. We also emphasized that our \setpush is proposed to efficiently estimate single-node PageRank specifically on undirected graphs. Please refer to the Abstract for details. 

    \item In the Introduction, we added a paragraph entitled ``Single-Node PageRank Computation on Undirected Graphs". In this paragraph, we illustrated the significance and necessity to estimate a single node's PageRank on undirected graphs from both theoretical and practical aspects. Please refer to Section~\ref{sec:intro} for details. 

    \item At the end of the Introduction, we summarized our major contributions into three points. In particular, in the first point, we provided Table~\ref{tbl:comparison} to show the theoretical improvements of our \setpush over existing methods for the single-node PageRank computation on undirected graphs. Moreover, in the third point of our contributions, we presented the high-level idea on how to utilize the theoretical properties of PageRank scores on undirected graphs in the development of our \setpush. 
\end{itemize}

\begin{figure}[t]
\centering
\begin{tabular}{c}
\hspace{-3mm}\includegraphics[width=80mm,trim=0 0 0 0,clip]{./Figs/example_undirected.png}
\end{tabular}
\vspace{-4mm}
%\caption{A toy example for the differences between single-node PageRank computations on undirected and directed graphs. }
\caption{A toy example for illustrating the hardness of estimating single-node PageRank on directed graphs. }
\label{fig:example_undirected}
\vspace{-4mm}
\end{figure}


%Based on the above observations, in this paper, we focus on the problem of single-node PageRank computation on undirected graphs, and achieve a better complexity result than the existing best result on undirected graphs. 
Note that our \setpush is developed specifically on undirected graphs. And we leave open the problem of whether the complexity bounds for estimating single-node PageRank on directed graphs can be further improved. 
%We leave open the problem of whether our \setpush can be expected
%Although our \setpush is proposed specifically on undirected graphs, we provide some comments here on the problem of single-node PageRank computation on directed graphs. 
%On the other hand, improving the complexity of single-node PageRank computation on directed graphs is another non-trivial problem. 
%Such equality implicitly bounds the value of $\vpi_u(t)$ for those high-degree nodes $u$. In other words, given a target node $t$, the value of $\vpi_u(t)$ is relatively small if $d_u$ is large. 
%differences between single-node PageRank computations on undirected and directed graphs. 
%provides a toy example to illustrate the differences between single-node PageRank computations on undirected and directed graphs. 
To see the hardness of the problem intuitively, we provide a toy example in Figure~\ref{fig:example_undirected}. 
Consider node $u_1$ in the left undirected graph with $d_{u_1}=\Theta(n)$. The transition probability from node $u_1$ to $t$ is $\Theta\left(\frac{1}{n}\right)$, and thus $\vpi_{u_1}(t)$ becomes $O\left(\frac{1}{n}\right)$. Therefore, if we conduct a backward push operation from node $t$, the probability mass reversely transferred from $t$ to $u$ is tiny. And the reverse propagation method can just stop after the first backward push operation as every $\vpi_u(t)$ for $\forall u\in N(t)$ turns out to be small. In comparison, consider the backward push operation from node $t$ in the right-side directed graph of Figure~\ref{fig:example_undirected}. The probability mass transferred from $t$ to every $u \in N_{in}(t)$ is significant since $d_{out}(u)=1$. Here $N_{in}(t)$ denotes the in-neighbor set of node $t$, and $d_{out}(u)$ denotes the out-degree of node $u$. As a result, the value of every $\vpi_u(t)$ is still large enough to conduct a new backward push operation from $u$. We note that $d_{in}(u)=\Theta(n)$ for every $u\in N_{in}(t)$, where $d_{in}(u)$ denotes the in-degree of node $u$. As a consequence, the time cost spent in the right directed graph is $\Theta(n^2)$, while we only require $\Theta(n)$ to estimate $\vpi(t)$ in the left undirected graph. %We leave open the question of whether the complexity of PageRank computation on directed graphs can be improved. 

The toy example given in Figure~\ref{fig:example_undirected} illustrates the hardness of estimating single-node PageRank on directed graphs. In the meanwhile, this toy example also reflects there indeed exist several important properties held by PageRank values on undirected graphs. At a high level, recall that the following equation (also given in Equation~\eqref{eqn:birectional_ppr}) holds for all nodes $u$ and $t$ in an undirected graph $G$: 
\begin{align*}
\vpi_u(t) \cdot d_u = \vpi_t(u) \cdot d_t. 
\end{align*}
%However, most of (if not all) existing methods fail to make fully use of this property, and incur large query time complexity both on directed and undirected graphs. 
%In this paper, we design the \setpush algorithm based on the above equation, and successfully achieve a better complexity result for single-node PageRank computation on undirected graphs. Specifically, we note that 
This equation actually implies the value of $\vpi_u(t)$ would not be extremely large if $d_u$ is large. We argue that this property is pretty crucial and should be highly valued when developing algorithms on undirected graphs. However, existing methods do not pay enough attention to this point, which leads to suboptimal complexity results and motivates us to contribute some improvements on this problem.  
%bounds the value of $\vpi_u(t)$ for those high-degree nodes $u$. In other words, given a target node $t$, the value of $\vpi_u(t)$ is relatively small if $d_u$ is large. 

%can be computed by $\vpi(t)=\frac{1}{n}\sum_{u\in V}\vpi_u(t)=\frac{1}{n}\sum_{u\in V}\frac{d_t}{d_u}\vpi_t(u)$. Thus, we no longer need to simulate $\alpha$-random walks from a uniformly selected source node $s$ for estimating the value of $\vpi_u(t)$ for every $u\in V$. Instead, we can propagate probability mass from node $t$ forward to its neighbors. As a result, we are able to break the lower bound $O\left(\frac{1}{\vpi(t)}\right)$ of the Monte-Carlo method, and achieve a better complexity compared to the Monte-Carlo method and all hybrid methods including a Monte-Carlo phase on undirected graphs. 



%In summary, existing methods for single-node PageRank computation mainly focus on directed graphs, while incur large time complexity due to the hardness of the problem. On the other hand, estimating single-node PageRank on undirected graphs is still of great importance from both practical and theoretical aspects. The PageRank scores on undirected graphs also have several unique properties, which are not fully utilized by existing methods. Motivated by the above issues, we 

\begin{comment}


revised the abstract and introduction of this paper to highlight this point. 
%in our contributions presented in the Introduction of the revised paper. 

Note that the three methods, LocalPush~\cite{lofgren2013personalized}, FastPPR~\cite{lofgren2014FastPPR}, and BiPPR~\cite{lofgren2016BiPPR}, are originally proposed on directed graphs. However, they cannot offer the worst-case guarantee on directed graphs without considering a uniform random choice of the target node. For an arbitrary target node, meaningful complexity bounds of the three methods can only be derived on undirected graphs (as listed in Table~\ref{tbl:comparison}). On the other hand, 

to our knowledge, the best complexity results achieved by existing methods on undirected graphs turn out to be the complexities of FastPPR, BiPPR and \sublinear, which one is the best determined by the specific values of $d, d_{\max}$ and $d_t$. However, the three methods are originally proposed on directed graphs, which reflects that existing methods do not make fully use of the properties of PageRank on undirected graphs. 
The two points mentioned above motivate us to study the problem of single-node PageRank computation on undirected graphs. To be more specific, we think the necessity to study the single-node PageRank computation problem on undirected graphs mainly come from two aspects. %Specifically, our motivations mainly come from two aspects: %The necessity is two-fold: 


First, from the theoretical aspect, some important properties of PageRank (or Personalized PageRank (PPR)) only hold on undirected graphs. For example, as shown in Equation~\eqref{eqn:birectional_ppr}, the following equation holds for all nodes $u$ and $t$ in an undirected graph $G$: 
\begin{align*}
\vpi_u(t) \cdot d_u = \vpi_t(u) \cdot d_t. 
\end{align*}
However, most of (if not all) existing methods fail to make fully use of this property, and incur large query time complexity both on directed and undirected graphs. 
In this paper, we design the \setpush algorithm based on the above equation, and successfully achieve a better complexity result for single-node PageRank computation on undirected graphs. Specifically, we note that the above equation implicitly implies $\vpi(t)$ can be computed by $\vpi(t)=\frac{1}{n}\sum_{u\in V}\vpi_u(t)=\frac{1}{n}\sum_{u\in V}\frac{d_t}{d_u}\vpi_t(u)$. Thus, we no longer need to simulate $\alpha$-random walks from a uniformly selected source node $s$ for estimating the value of $\vpi_u(t)$ for every $u\in V$. Instead, we can propagate probability mass from node $t$ forward to its neighbors. As a result, we are able to break the lower bound $O\left(\frac{1}{\vpi(t)}\right)$ of the Monte-Carlo method, and achieve a better complexity compared to the Monte-Carlo method and all hybrid methods including a Monte-Carlo phase on undirected graphs. 





Second, from the practical aspect, the problem of single-node PageRank computation on undirected graphs is of great importance. Many downstream graph mining and learning tasks are only defined on undirected graphs. All input directed graphs are required to be converted to undirected graphs. For example, in the scenario of local clustering, the well-adopted {\em conductance} metric to measure the quality of identified clusters is defined on undirected graphs. Thus, %most of (if not all) local clustering algorithms are only for undirected graphs. Among them, 
a celebrated local clustering method~\cite{FOCS06_FS} employ the Personalized PageRank vector computed on undirected graphs to find local clusters. Moreover, Graph Neural Networks (GNNs) have drawn increasing attention in recent years. A plethora of GNN models leverage PageRank computation to propagate node features~\cite{klicpera2019APPNP, Bojchevski2020PPRGo,Chen2020GCNII}. Because the graph Laplacian matrix for feature propagation is only applicable to undirected graphs, this line of research invokes PageRank computation algorithms only on undirected graphs. 





% On the other hand, a number of existing algorithms do not offer any worst-case guarantee on directed graphs without considering a uniform random choice of the target node. For example, the canonical reverse exploration algorithm, LocalPush~\cite{lofgren2013personalized}, requires $O\left(n\cdot \left(\sum_{v\in V} \vpi_{v}(t)\cdot d_v\right)\right)$ time cost for estimating an arbitrary target node $t$'s PageRank on directed graphs. Such complexity can be rewritten as a meaning bound $O(n\cdot d_t)$ only on undirected graphs, by applying the property of PPR on undirected graphs: $\vpi_v(t) \cdot d_v = \vpi_t(v) \cdot d_t$. The same problem also holds in the hybrid methods, FastPPR~\cite{lofgren2014FastPPR} and BiPPR~\cite{lofgren2016BiPPR}, which include a reverse propagation phase in the algorithm. 
%As a consequence, although these methods are originally proposed for single-node PageRank computation on directed graphs, their complexity bounds are only applicable to undirected graphs with an arbitrary target node. 
\end{comment}




\subsection*{Reviewer \#2} \label{sec:r2}
\review{\bf W1}: {\em Table 2 is not centered like Table 1, which I think is better centered. } 

\header{\bf Response: } Thanks for the suggestion. We centered the contents in Table 2 as advised. 


\review{\bf W2}: {\em Add description of hyperparameters’ setting. } 

\header{\bf Response: } {\rev TODO}


\review{\bf W3}: {\em Add experiments for parameter sensitivity of the algorithm on datasets. } 

\header{\bf Response: } {\rev TODO}




\subsection*{Reviewer \#4} \label{sec:r4}

\begin{table*} [t]
%\vspace{-4mm}
\centering
\renewcommand{\arraystretch}{1.4}
%\begin{small}
\tblcapup
\caption{Comparison of algorithms for estimating single-node PageRank on undirected graphs with constant relative error and constant success probability. The complexity results marked with $\star$ are only applicable on undirected graphs. 
%In the last column, we list the ratio of our \setpush's query time complexity to every baseline's time complexity. The smaller the ratio is, the larger improvement \setpush performs over the baseline method. 
}\label{tbl:comparison_rev}
\vspace{-2mm}
%\resizebox{0.9\linewidth}{!}{%
%\resizebox{1\linewidth}{!}{
%\tblcapdown
%p{2.3in}
\begin{tabular} 
%{|l|p{2.3in}|} \hline
{|P{3.5cm}|c@{\hspace{+1mm}}|@{\hspace{+1mm}}c@{\hspace{+1mm}}|@{\hspace{+1mm}}P{6.3cm}|} \hline
{\bf Query Time Complexity} & \multirow{2}*{\bf Baseline Methods} &  {\bf Query Time Complexities} & {\bf {Improvement of \setpush over Baselines}} \\ 
{\bf of Our \setpush} & & {\bf of Baseline Methods} & (the larger, the better) \\ \hline
%~& & & (the time) \\ \hline
\multirow{7}*{$\tilde{O}\left(\min\left\{d_t, \sqrt{m}\right\}\right) \star$} & The Power Method~\cite{page1999pagerank} & $\tilde{O}(m)$ & $\max \left\{ m / d_t, \sqrt{m} \right\}$  \\  \cline{2-4}
& Monte-Carlo~\cite{fogaras2005MC} & $\tilde{O}(n)$ & $\max \left\{n/d_t,  \sqrt{n/\davg} \right\}$ \\ \cline{2-4}
%LocalPush~\cite{andersen2007contribution} & $\tilde{O}\left(n\cdot d_t\right)$ \\ \hline
& LocalPush~\cite{lofgren2013personalized} & $\tilde{O}\left(\min\left\{n\cdot d_t, m\right\}\right) \star$ & $\sqrt{m}$ \\ \cline{2-4}
&  RBS~\cite{wang2020RBS} & $\tilde{O}\left(n\right)$ & $\max \left\{n / d_t, \sqrt{n/\davg} \right\}$ \\ \cline{2-4}
& FastPPR~\cite{lofgren2014FastPPR} &  $\tilde{O}\left(\sqrt{n\cdot d_t}\right) \star$ & $\max \left\{\sqrt{n / d_t}, \sqrt{d_t / d}\right\}$ \\ \cline{2-4}
& BiPPR~\cite{lofgren2016BiPPR} & $\tilde{O}\left(\sqrt{n\cdot d_t}\right) \star$ & $\max \left\{\sqrt{n / d_t}, \sqrt{d_t / d}\right\}$ \\ \cline{2-4}
%\rule{0pt}{14pt} Bressan-PageRank~\cite{bressan2018sublinear} & {$\tilde{O}\left(\min\left\{\frac{m^{2/3}\Delta^{1/3}}{d^{1/2}}, \frac{m^{4/5}}{d^{3/5}} \right\}\right)$}\\[1ex] \hline
& \sublinear~\cite{bressan2018sublinear} & {$\tilde{O}\left(\min\left\{\frac{m^{2/3}\cdot \dmax^{1/3}}{\davg^{2/3}}, \frac{m^{4/5}}{\davg^{3/5}} \right\}\right)$} 
& $\max \left\{\min \left\{\frac{n^{\frac{2}{3}}\cdot d_{\max}^{1/3}}{d_t}, \frac{n^{\frac{4}{5}} \cdot d^{\frac{1}{5}}}{d_t}\right\}, \min\left\{\frac{n^{\frac{1}{6}}\cdot d_{\max}^{1/3}}{d^{\frac{1}{2}}}, \frac{n^{\frac{3}{10}}}{d^{\frac{3}{10}}}\right\}\right\}$\\ \hline
%\rule{0pt}{14pt}$\mymathhl{\text{\setpush(Ours)}}$ & $\mymathhl{\tilde{O}(\min\left\{d_t, \sqrt{m}\right\})}$ \\[1ex] \hline
%& \setpush(Ours) & $\tilde{O}\left(\min\left\{d_t, \sqrt{m}\right\}\right)$ & \\ \hline
\end{tabular}
%}
\vspace{-3mm}
%\end{small}
\end{table*}


\review{\bf W1}: {\em The contribution of this work seems not obviously. There exist several algorithms to solve the single node PageRank problem. It is necessary to show the significant improvement and advantages of the proposed algorithms against existing methods in this paper. } 

\header{\bf Response: } Thanks for the advice! We made the following modifications in the revised paper to highlight our contributions. 
%We revised the Introduction and summarized our contribution into three points
%re-summarized our contributions in the Introduction to highlight the major points. For reference, we present a brief summary (with some additional illustrations) on our core contributions in the following. %Please refer to Section~\ref{subsec:contribution} for details. 
%A more comprehensive version can be found in Section~\ref{subsec:contribution}. 
%First, we re-summarized our contributions in the Introduction into three points. 

First of all, in the Introduction of the revised paper (see Section~\ref{subsec:contribution}), we explicitly listed the theoretical improvements of our \setpush over existing methods on undirected graphs. Specifically, as shown in Table~\ref{tbl:comparison}, the expected time complexity of our \setpush is no worse than that of any existing method on undirected graphs. In particular, as given in the last column of Table~\ref{tbl:comparison}, our \setpush improves FastPPR~\cite{lofgren2014FastPPR} and BiPPR~\cite{lofgren2016BiPPR} by a factor of $\varphi=\max \left\{\sqrt{n/{d_t}}, \sqrt{d_t / \davg }\right\}$, and improves the \sublinear method~\cite{bressan2018sublinear} by 
\begin{align*}
\varphi=\max \left\{\min \left\{\frac{n^{\frac{2}{3}}\cdot d_{\max}^{1/3}}{d_t}, \frac{n^{\frac{4}{5}} \cdot d^{\frac{1}{5}}}{d_t}\right\}, \min\left\{\frac{n^{\frac{1}{6}}\cdot d_{\max}^{1/3}}{d^{\frac{1}{2}}}, \frac{n^{\frac{3}{10}}}{d^{\frac{3}{10}}}\right\}\right\}, 
\end{align*}
where $\davg$ and $\dmax$ denote the average and maximum node degree of the graph, respectively. Note that FastPPR, BiPPR and the \sublinear method achieve the best complexity results among existing methods for deriving a $(c, p_f)$-approximation of $\vpi(t)$ on undirected graphs (which one is the best depends on the specific values of $d_t$, $\davg$ and $\dmax$). Unless on a complete graph where $\davg=n$, the improvements $\varphi$ of \setpush over FastPPR, BiPPR, and \sublinear are all strictly larger than $1$, which means the expected time complexity of \setpush is asymptotically better than that of any existing method. 
%Furthermore, as illustrated in our response to the D2 point given below, 
Even on a complete graph, in which case $\varphi=1$, the complexity of \setpush is no worse than those of FastPPR, BiPPR, and \sublinear, and still better than those of LocalPush, Monte-Carlo, and the power method. 


It's worth to mention that complete graphs are severely rare in real-world applications. Actually, it was empirically observed that most real-world networks are scale-free and follow power-law degree distribution with the power-law exponent $2\le \gamma \le 3$~\cite{barabasi2013network, wang2017fora, wei2019prsim, lofgren2013personalized}. In such scale-free graph, the average node degree is $\davg=m/n=O(\log{n})$~\cite{wang2017fora}, 
%In particular, when the input graphs are scale-free with
%consider a scale-free graph where $\davg=m/n=O(\log{n})$~\cite{wang2017fora} and $\dmax=O(n)$ due to the existence of hub nodes. 
in which case our \setpush significantly outperforms existing methods in terms of computational time complexity. In the meantime, when the target node $t$'s degree is small (e.g., $d_t=O(1)$), the improvement of our \setpush over existing methods is also significant. Specifically, we have the following observations. 
\begin{itemize}
\item For the power method~\cite{page1999pagerank}, our \setpush improves it by a factor of $\tilde{O}\left(\max\left\{\frac{m}{d_t}, \sqrt{m}\right\}\right)$. In particular, when $d_t=O(1)$, \setpush significantly outperforms the power method by an $\tilde{O}\left(m\right)$ factor. 

\item For the Monte-Carlo method~\cite{fogaras2005MC}, our \setpush improves it by a factor of $\tilde{O}\left(\frac{n}{d_t}, \sqrt{\frac{n}{\davg}}\right)$. When $d_t=O(1)$, the improvement of \setpush over the Monte-Carlo method turns out to be a $\tilde{O}(n)$ factor. On the other hand, considering a scale-free networks with $\davg=O(\log{n})$, our \setpush significantly at least improves the Monte-Carlo method by a factor of $\tilde{O}\left(\sqrt{\frac{n}{\log{n}}}\right)$. 

\item For the LocalPush method~\cite{lofgren2013personalized}, our \setpush significantly outperforms it by an $\tilde{O}\left(\sqrt{m}\right)$ factor. 
    
\item For FastPPR~\cite{lofgren2014FastPPR} and BiPPR~\cite{lofgren2016BiPPR}, our \setpush improves both of the two methods by a factor of $\tilde{O}\left(\sqrt{\frac{n}{d_t}}, \sqrt{\frac{d_t}{\davg}}\right)$. In particular, on a scale-free graph with $\davg=O\left(\log{n}\right)$, \setpush outperforms the two methods by a factor of at least $\tilde{O}\left(\left(\frac{n}{\log{n}}\right)^{\frac{1}{4}}\right)$. On the other hand, when $d_t=O(1)$, \setpush significantly improves the two methods by a $\tilde{O}\left(\sqrt{n}\right)$ factor. 
%improves over FastPPR and BiPPR by at least $\max \left\{\sqrt{\frac{n}{\log{n}}}, \sqrt{\frac{}{}}\right\}$. 

\item For the \sublinear method~\cite{bressan2018sublinear}, our \setpush outperforms it by a factor of $\tilde{O}\left(\max \left\{\min \left\{\frac{n^{\frac{2}{3}}\cdot d_{\max}^{1/3}}{d_t}, \frac{n^{\frac{4}{5}} \cdot d^{\frac{1}{5}}}{d_t}\right\}, \min\left\{\frac{n^{\frac{1}{6}}\cdot d_{\max}^{1/3}}{d^{\frac{1}{2}}}, \frac{n^{\frac{3}{10}}}{d^{\frac{3}{10}}}\right\}\right\}\right)$. In particular, on scale-free networks with $d=O(\log{n})$, \setpush improves over the \sublinear method by at least a $\tilde{O}\left(\left(\frac{n}{\log{n}}\right)^{3 \over 10}\right)$ factor. Alternatively, when the given target node $t$ is a low-degree node (e.g., $d_t=O(1)$ is a constant), our \setpush significantly outperforms the \sublinear method by a factor of at least $\tilde{O}\left(\min \left\{n^{\frac{2}{3}}\cdot d_{\max}^{1/3}, n^{\frac{4}{5}}\cdot d^{\frac{1}{5}}\right\}\right)$. 
\end{itemize}


Moreover, in Section~\ref{subsec:reasonswhy} of the revised paper, we also elaborated on the reasons why existing methods cannot achieve the $\tilde{O}\left(\min\left\{d_t, \sqrt{m}\right\}\right)$ complexity result of \setpush on undirected graphs. And we attributed the theoretical improvements achieved by our \setpush to two points of contribution given below (also presented in Section~\ref{subsec:contribution} and Section~\ref{subsec:highlevelidea} of the revised paper). 
\begin{itemize}
    \item The reverse exploration method (e.g., LocalPush~\cite{lofgren2013personalized}) and most of the hybrid method (e.g., FastPPR~\cite{lofgren2014FastPPR} and BiPPR~\cite{lofgren2016BiPPR}) adopt the vanilla backward push operations to reversely propagate the probability mass from the target node to its ancestors. However, the backward push operation (e.g., at node $u$) has to touch every neighbor of $u$ to push the probability mass, which leads to an $O(d_u)$ lower bound for the time cost of the backward push at $u$. In our \setpush, we propose a novel push operation, which simultaneously mixes the deterministic backward push and randomized Monte-Carlo sampling in one atomic step. Benefit from the novel push operation, we deterministically cost $O(d_u)$ time only at the node $u$ with small $d_u$, and randomly sample a fraction of $u$'s neighbors to push probability mass if $d_u$ is large. As a result, we successfully remove the $O(d_u)$ term introduced by the vanilla push operation at node $u$, and achieve a superior time complexity over the reverse exploration method (e.g., LocalPush) and most of the hybrid methods (e.g., FastPPR and BiPPR). 

    \item Considering the problem of single-node PageRank computation, existing methods mainly focus on directed graphs, and fail to make full use of the properties held by PageRank values on undirected graphs. In comparison, our \setpush algorithm is designed specifically on undirected graphs. We elaborately leverage the properties of PageRank on undirected graphs to achieve superior time complexity result. Specifically, we note that the canonical Monte-Carlo sampling admits an $\Omega\left(\frac{1}{\vpi(t)}\right)$ lower bound for deriving a $(c, p_f)$-approximation of $\vpi(t)$ even on undirected graphs. Worse still, by the definition formula of PageRank, the initial probability distribution of simulating $\alpha$-random walks is $\frac{1}{n}\cdot \bm{1}=\left(\frac{1}{n}, \frac{1}{n}, \ldots, \frac{1}{n}\right)$. Therefore, in the worst-case scenario where $\vpi(t)=O\left(\frac{1}{n}\right)$, the Monte-Carlo method requires $\Omega(n)$ $\alpha$-random walks to hit node $t$ at least once. However, on undirected graphs, it is actually no longer necessary to simulate $\alpha$-random walks from a uniformly selected source node $s$. Inspired by this observation, we successfully break the lower bound $O\left(\frac{1}{\vpi(t)}\right)$ of Monte-Carlo sampling with non-trivial analyses. As a consequence, our \setpush achieves a superior complexity result compared to all existing methods that include Monte-Carlo sampling phase (e.g., the Monte-Carlo method~\cite{fogaras2005MC}, FastPPR~\cite{lofgren2014FastPPR}, BiPPR~\cite{lofgren2016BiPPR}, and the \sublinear method~\cite{bressan2018sublinear}). 
    
\end{itemize}







\review{\bf W2}: {\em The descriptions of experimental results and the figures are not one-to-one corresponded. It seems need to be double-checked. } 

\header{\bf Response: } Thanks for the suggestion. We revised the experimental descriptions as advised. Please refer to Section~\ref{sec:exp} for details. 


\review{\bf W3}: {\em It will be better to provide more experiments to verify the performance of the proposed algorithm. Details are in the detailed comments. } 

\header{\bf Response: } {\rev TODO}



\review{\bf D1}: {\em The paper proposes a new SetPush algorithm to solve the single node PageRank estimating problem which also provides detailed theoretical analysis. However, the superiority of the proposed algorithm against the existing methods is not shown significantly in practice. For example, the existing SubgraphPush algorithms seems can provide a similar or better query time on some datasets (Figure 6). } 

\header{\bf Response: } {\rev TODO}



\review{\bf D2}: {\em Since I have checked that the query time of SubgraphPush presented in~\cite{bressan2018sublinear} is $O\left(\min\left\{\frac{m^{2/3} d^{1/3}_{max}}{d^{2/3}}, \frac{m^{4/5}}{d^{3/5}}\right\} \right)$, which is different with that reported in Table 1 of this paper, it will be better to explain it. } 

\header{\bf Response: } The expected time complexity of the SubgraphPush method~\cite{bressan2018sublinear} is $\tilde{O}\left(\min\left\{\frac{m^{2/3} d^{1/3}_{max}}{d^{2/3}}, \frac{m^{4/5}}{d^{3/5}}\right\} \right)$. The complexity of SubgraphPush listed in Table~\ref{tbl:comparison} in the original manuscript is incorrect. We sincerely thank the reviewer for pointing out this typo, and we are sorry for this discrepancy. We have corrected this typo in the revised paper. Please refer to Table~\ref{tbl:comparison} for details (also shown in Table~\ref{tbl:comparison_rev} given below for convenience). 

Nonetheless, our \setpush STILL achieves superior query efficiency over the \sublinear method~\cite{bressan2018sublinear} for deriving a $(c,p_f)$-approximation of $\vpi(t)$ on undirected graphs (defined in Definition~\ref{def:problem}). Specifically, our \setpush improves over the \sublinear method by a factor of: 
\begin{align*}
\varphi=\max \left\{\min \left\{\frac{n^{\frac{2}{3}}\cdot d_{\max}^{1/3}}{d_t}, \frac{n^{\frac{4}{5}} \cdot \davg^{\frac{1}{5}}}{d_t}\right\}, \min\left\{\frac{n^{\frac{1}{6}}\cdot d_{\max}^{1/3}}{\davg^{\frac{1}{2}}}, \frac{n^{\frac{3}{10}}}{\davg^{\frac{3}{10}}}\right\}\right\},     
\end{align*}
where $\dmax$ and $\davg$ denote the maximum and average node degree of the graph $G$, respectively. A detailed illustration to derive the value of $\varphi$ can be found in our response to D6 of Reviewer \#5. We note that the factor $\varphi$ is asymptotically larger than $1$ unless $\davg=n$. Thus, the expected query time complexity of \setpush is {\em asymptotically better} than that of \sublinear unless $\davg=n$. Even when $\davg=n$ (i.e., on a complete graph), in which case $\varphi=1$, the complexity of \setpush is no worse than that of \sublinear. Please refer to our response to the W1 point in this section for detailed illustrations on our contributions and the superiority of \setpush over existing methods. 

%Note that a complete graph is severely rare in real-world applications. Actually, it was empirically observed that most real-world networks are scale-free and follow power-law degree distribution with the power-law exponent $2\le \gamma \le 3$~\cite{barabasi2013network, wang2017fora, wei2019prsim, lofgren2013personalized}. In such scale-free graph, the average node degree is $\davg=m/n=O(\log{n})$~\cite{wang2017fora}, %In particular, when the input graphs are scale-free with %consider a scale-free graph where $\davg=m/n=O(\log{n})$~\cite{wang2017fora} and $\dmax=O(n)$ due to the existence of hub nodes. 
%and thus, our \setpush improves over the \sublinear method by at least $\left(\frac{n}{\log{n}}\right)^{3 \over 10}$. %It was empirically observed that most real-world networks are scale-free and follow power-law degree distribution. 
%Furthermore, if the given target node $t$ is a low-degree node (e.g., $d_t=O(1)$ is a constant), our \setpush significantly outperforms the \sublinear method by at least $\min \left\{n^{\frac{2}{3}}\cdot d_{\max}^{1/3}, n^{\frac{4}{5}}\cdot d^{\frac{1}{5}}\right\}$, whether or not on scale-free graphs. 



\review{\bf D3}: {\em As shown in Table~\ref{tbl:comparison}, the existing FastPPR, BiPPR and SubgraphPush algorithms have the better performance than others. However, the paper only compares the proposed algorithm to SubgraphPush algorithm. It is necessary to evaluate the query time by comparing with FastPPR or BiPPR. } 

\header{\bf Response: } {\rev TODO}


\review{\bf D4.1}: {\em It will be better to show how the query time changes with $d_t$ increasing to illustrate the superiority of the proposed algorithms.} 

\header{\bf Response: } {\rev TODO}


\review{\bf D4.2}: {\em In Figure 6, SubgraphPush provides better results than SetPush on YT and OL datasets. It will be better to explain the reason.} 

\header{\bf Response: } {\rev TODO}


\review{\bf D4.3}: {\em Page 12, Experimental Results, Figure 3 and Figure 6 -> Figure 3 and Figure 4. It is necessary to clearly state that the omitted result on Friendster in Figure 3 is the MC algorithm. The omitted results on Friendster in Figure 5 are LocalPush and MC.} 

\header{\bf Response: } {\rev TODO}




\subsection*{Reviewer \#5} \label{sec:r5}

\review{\bf W1}: {\em The application/motivation for estimating the PageRank value of a single node is unclear.} 

\review{\bf D1}: {\em It is unclear what are the applications of estimating the PageRank value of a single node.} 

\header{\bf Response to W1 and D1: } Thanks for pointing out this issue. We added detailed descriptions to elaborate on the applications and motivations for estimating a single node's PageRank value. Please refer to the Introduction of the revised paper for details. 

Briefly speaking, we first listed multiple application scenarios of PageRank computation in the Introduction, including web search, social networks, recommender systems, databases, as well as biology, chemistry, neuroscience and etc. Then we provided a concrete example in which case all we need is an approximation of one or a few nodes' PageRank scores. Specifically, consider a data mining task that we are required to observe the changes in the importance of a few popular websites (e.g., the top-10 most important websites ranked last year). In this case, we will frequently ask for the PageRank scores of the 10 websites given the fact that websites' global importance can be reflected from their PageRank scores. Notably, it would be prohibitively slow to score all nodes in the graph every time, especially on large-scale graphs with millions or even billions of nodes and edges. Therefore, an ideal solution for such case is a {\em local} algorithm, which is able to efficiently return the target node's approximation scores by only exploring a small fraction of graph edges around the target node. However, as pointed out by~\cite{bressan2018sublinear}, most of existing approaches require an $\Omega(n)$ time complexity for single-node PageRank computation. %We also illustrate the limitations of existing methods in Section~\ref{sec:algorithm}. 
Thus, designing an efficient local algorithm for single-node PageRank computation remains a challenging task. This motivates us to study the problem of single-node PageRank computation from the practical aspect. 

Furthermore, from the theoretical aspect, we note that the query time complexity of single-node PageRank is related to several graph analysis problems. For example, as we illustrate in Section~\ref{sec:pre} (i.e., Equation~\eqref{eqn:PageRank_PPR}), node $t$'s PageRank is equal to the average over all nodes $u$ of $\vpi_u(t)$, where $\vpi_u(t)$ denotes the Personalized PageRank (PPR) of node $t$ with respect to node $u$. We call the problem single-target PPR queries, in which we ask for $\vpi_u(t)$ of every node $u\in V$. Therefore, 
any theoretical insight for single-node PageRank computation may be extended to solve the problem of single-target PPR queries. 
Additionally, as proved in~\cite{bressan2018sublinear}, the algorithm for single-node PageRank computation proposed in~\cite{bressan2018sublinear} also holds for Heat Kernel PageRank (HKPR). All of the above demonstrate that the problem of single-node PageRank computation is a primitive of theoretical interest. 


\review{\bf W2, D2}: {\em It seems that the proposed algorithm does not work on directed graphs or absolute error estimation.} 

\header{\bf Response: } Our \setpush algorithm is proposed to efficiently estimate single-node PageRank within constant relative error on undirected graphs. The complexity of $\tilde{O}\left(\min \left\{d_t, \sqrt{m}\right\}\right)$ achieved by our \setpush is only applicable to undirected graphs with the relative error constraint. 

It is worth to mention that the problem of estimating single-node PageRank on undirected graphs is of great importance from both practical and theoretical aspects (see the Introduction for details). Moreover, there exist some valuable properties of PageRank scores only held on undirected graphs (see our response to the Meta-Reviewer for details). However, existing methods do not pay enough attention to these properties, and fail to make full use of these properties to design efficient algorithms on undirected graphs. As a result, the best complexity bound for estimating single-node PageRank on undirected graphs is achieved by the algorithm originally proposed on directed graphs, with a large theoretical gap to be further improved. On the other hand, improving the complexity of single-node PageRank computation on directed graphs is a non-trivial problem. 
We provided a toy example to intuitively illustrate the hardness in our response to the Meta-Reviewer. 
%on the difference between single-node PageRank computations on undirected and directed graphs . 
As a result, although most of existing methods mainly focus on directed graphs, some of them even can not offer worst-case guarantee on directed graphs without considering a uniform random choice of the target node. For these methods (e.g., LocalPush~\cite{lofgren2013personalized}, FastPPR~\cite{lofgren2014FastPPR}, and BiPPR~\cite{lofgren2016BiPPR}), meaningful complexity bounds can only be derived on undirected graphs when we consider an arbitrary target node. 

Based on the above observations, in this paper, we focus on the problem of single-node PageRank computation on undirected graphs. We propose a novel algorithm \setpush, in which we design a novel push operation and elaborately make use of the theoretical properties held by PageRank scores on undirected graphs. As a consequence, our \setpush outperforms existing methods on undirected graphs in terms of expected computational time complexity. %We presented a elaborated description to illustrate the above issues in the Introduction of the revised paper, and in our response to the Meta-Reviewer. Please refer these contents for more details. 
%In the Introduction, we added a detailed illustration on the importance and pressing demand to study the problem of single-node PageRank computation on undirected graphs. And in our response to the Meta-Reviewer, we elaborate on the hardness of improving the time complexity for the single-node PageRank computation on directed graphs. Please refer to Section~\ref{sec:intro} and our response to the Meta-Reviewer for details. 

%The major reasons are listed as below. 
%\begin{itemize}
%\item First, from the practical aspect, many downstream graph mining and learning tasks are only defined on undirected graphs. All input directed graphs are required to be converted to undirected graphs. For example, in the scenario of local clustering, the well-adopted {\em conductance} metric to measure the the quality of identified clusters is defined on undirected graphs. Thus, %most of (if not all) local clustering algorithms are only for undirected graphs. Among them, 
%a celebrated local clustering method~\cite{FOCS06_FS} employ the Personalized PageRank vector computed on undirected graphs to find local clusters. Moreover, Graph Neural Networks (GNNs) have drawn increasing attention in recent years. A plethora of GNN models leverage PageRank computation to propagate node features~\cite{klicpera2019APPNP, Bojchevski2020PPRGo,Chen2020GCNII}. Because the graph Laplacian matrix for feature propagation is only applicable to undirected graphs, this line of research invokes PageRank computation algorithms only on undirected graphs. 

%\item Second, from the theoretical aspect, existing methods for single-node PageRank computation mainly focus on directed graphs. %which, however, incur large query time complexity despite decades of efforts due to the hardness. In this paper, we settle for a slightly less ambitious target to efficiently estimate single-node PageRank {\em on undirected graphs}. However, a number of existing algorithms do not offer any worst-case guarantee on directed graphs without considering a uniform random choice of the target node. For these methods, meaningful complexity bounds  can only be derived on undirected graphs when we consider an arbitrary target node (e.g., the LocalPush~\cite{lofgren2013personalized}, FastPPR~\cite{lofgren2014FastPPR}, and BiPPR~\cite{lofgren2016BiPPR} methods as listed in Table~\ref{tbl:comparison}). 
%Note that the three methods, LocalPush~\cite{lofgren2013personalized}, FastPPR~\cite{lofgren2014FastPPR}, and BiPPR~\cite{lofgren2016BiPPR}, are originally proposed on directed graphs. However, they cannot offer the worst-case guarantee on directed graphs without considering a uniform random choice of the target node. 
%(as listed in Table~\ref{tbl:comparison}). 
%On the other hand, to our knowledge, the best complexity results for single-node PageRank computation on undirected graphs are achieved by FastPPR~\cite{lofgren2014FastPPR}, BiPPR~\cite{lofgren2016BiPPR} and \sublinear~\cite{bressan2018sublinear}. %(which one is the best determined by the specific values of $d, d_{\max}$ and $d_t$).
%However, the three methods are originally proposed on directed graphs. This reflects that existing methods do not fully utilize the properties of PageRank on undirected graphs, and leaves significant theoretical gaps to be improved on undirected graphs. %The two points mentioned above motivate us to study the problem of single-node PageRank computation on undirected graphs. 

    
%\end{itemize}




For the concern on the choice of approximation error metric, it is actually a well-adopted goal to estimate single-node PageRank (or single-target PPR, single-node HKPR, etc) under relative error in literature~\cite{bressan2018sublinear, lofgren2016BiPPR, lofgren2014FastPPR, wang2020RBS, yang2019TEA}. On the other hand, as pointed out in~\cite{dagum2000optimal}, for those small PageRank scores $\vpi(t)$, a good absolute error estimate is typically a poor approximation of $\vpi(t)$ in terms of relative error. Unfortunately, in an $n$-node graph, all except $o(n)$ nodes have small PageRank scores $O\left(\frac{1}{n}\right)$~\cite{bressan2018sublinear}. This means for almost every target node $t$ in the graph $G$, computing an estimate of $\vpi(t)$ under relative error is much harder than deriving a good absolute error estimate. Furthermore, as shown in~\cite{wang2020RBS}, the approximation algorithm under relative error can also be used to derive an absolute error estimate just with a slight modification, which, however, is beyond the scope of our paper. We leave this as our future work. 

%in this paper, we analyze the theoretical properties of our \setpush under relative error. 
%our \setpush may be extended to estimate single-node PageRank with absolute error. 

%Finally, we admit that it is an non-trivial problem to improve the complexity bound for the single-node PageRank computation on directed graphs. We leave open this problem as a future work presented in the Conclusion (see Section~\ref{sec:conclusion}). Please refer to our response to Meta-Reviewer for details. 



\review{\bf W3}: {\em Discussions on the applicability of the proposed new push operator to other PageRank estimation problems are not discussed.} 

\review{\bf D8}: {\em As the main idea is the new push operator (which actually is similar to the push operator used in RBS), it would be better to discuss the applicability of the new push operator to other PageRank estimation problems, such as PPR to a target node, single source PPR, and directed graphs. For example, can it replace the push operator used in LocalPush? } 


\header{\bf Response to W3 and D8: } 
%Thanks for the advice! Note that the superiority of \setpush mainly comes from two aspects. On one hand, we propose a novel push operation, which mixes the deterministic backward push and randomized Monte-Carlo sampling in one atomic step. In the new push operation (e.g., at node $u$), we do not need to touch every neighbor of $d_u$, and thus, improve the time complexity of the reverse exploration method. It's worth to mention that our push operation is in spirit to push operation adopted in RBS, but differs in one crucial aspect. That is, the sampling technique adopted in the push operation of RBS is non-independent, which results large variance for the single-node PageRank computation. In comparison, in the \setpush method, the increment of $\r_t^{(\ell)}$ for each $v\in V$ is independent with each other. As a consequence, the time complexity of our \setpush for estimating the single-node PageRank on undirected graphs is asymptotically better than that of the RBS method~\cite{wang2020RBS}. 

%On the other hand, we observe that there are several crucial properties held by the PageRank values on undirected graphs. However, existing methods do not pay enough attention to these properties, leading to suboptimal complexity results on undirected graphs. In our \setpush, we elaborately leverage these valuable properties, and successfully avoid the $O(n)$ time cost introduced by Monte-Carlo sampling in the worst-case scenario. 








\review{\bf D3}: {\em As the main contribution of the paper is the detailed theoretical analysis of the proposed push operator (and the resulting graph), a theoretical venue may be more suitable for this paper. } 

\header{\bf Response: } Thanks for the advice! However, we still believe the scope of the paper is highly relevant to the VLDB conference. The reasons can be summarized into three points given below. 
\begin{itemize}
\item In this paper, we focus on the problem of estimating single-node PageRank on undirected graphs. As we illustrated in the Introduction, PageRank is a highly important graph centrality metric, which is widely adopted in numerous real-world applications. Moreover, computing a single node's PageRank is also of great significance from both theoretical and practical aspects. Please refer to our response to the W1 point of Reviewer \#5 for more supporting details. Therefore, we believe the problem of single-node PageRank computation on undirected graphs is definitely of particular interest in the VLDB community

\item Motivated by the pressing need of efficient single-node PageRank algorithms on undirected graphs, we propose the \setpush algorithm, which achieves the best time complexity result among existing methods on undirected graphs. We theoretically prove the improvements of \setpush with non-trivial analysis, and illustrate the core advantages of our \setpush compared to other baselines. We also provide elaborated descriptions on the reasons why existing methods cannot achieve the complexity bound of \setpush. We believe the \setpush algorithm can bring some new ideas and theoretical insights to the VLDB community. 

\item Finally, we conduct comprehensive experiments on large-scale real-worlds datasets. Our experimental results demonstrate that our \setpush outperforms existing methods on undirected graphs in terms of query efficiency. 

\end{itemize}


\review{\bf D4}: {\em $c$ is ignored from the time complexity analysis. It will be better if the authors could also provide a version of the time complexity analysis with $c$ included; for example, what would the polynomial order of $c$ be? } 

\header{\bf Response: } Thanks for the advice. We included $\alpha, c$ and all logarithmic factors in the time complexity analysis. Please see Theorem~\ref{thm:finalcost_analysis} and its proof for details. 


\review{\bf D5}: {\em What are ignored by the $\tilde{O}$ notation is not mentioned in the paper? } 

\header{\bf Response: } $\tilde{O}$ is a commonly-used asymptotic notation and is widely adopted in literature (e.g., ~\cite{bressan2018sublinear, wang2020RBS, teng2016scalable}). Specifically, given a function $g(n)$, $\tilde{O}\left(g(n)\right)$ denotes the set of functions: 
\begin{align*}
\tilde{O}\left(g(n)\right)\hspace{-0.5mm}=\hspace{-0.5mm}\left\{f(n) \mid \exists\textit{~constant~} c \hspace{-0.5mm}>\hspace{-0.5mm} 0, \textit{such that~} f(n)\hspace{-0.5mm}=\hspace{-0.5mm}O\left(g(n)\hspace{-0.5mm} \cdot \hspace{-0.5mm} \log^c{n}\right)\right\}. 
\end{align*}
The above definition is presented in Section 1.2 of~\cite{teng2016scalable}. In other words, $\tilde{O}$ is a variant of the Big-Oh notation that ignores poly-logarithmic factors. For example, $n\log{n} = \tilde{O}(n)$. 
%, and $n^2 \log{n} \log{\log{n}}=\tilde{O}\left(n^2\right)$. 
%The $\tilde{O}$ notation is widely adopted in literature (e.g., ~\cite{bressan2018sublinear, wang2020RBS, teng2016scalable}) to make a . 
We explained the meaning of the $\tilde{O}$ notation in Table~\ref{tbl:def-notation}, and added more explanations on $\tilde{O}$ in the Introduction (see Section~\ref{subsec:contribution} for details). 



\review{\bf D6}: {\em In the Introduction, it is unclear why $\bar{d}^{1/5} \cdot n^{4/5}$ would be always no smaller than $d_t$. For example, what if $\bar{d}$ is small while $d_t$ is large? } 

\header{\bf Response: } Thanks for pointing out this. The expected time complexity of SubgraphPush~\cite{bressan2018sublinear} is $\tilde{O}\left(\min\left\{\frac{m^{2/3} d^{1/3}_{max}}{d^{2/3}}, \frac{m^{4/5}}{d^{3/5}}\right\} \right)$. The complexity of SubgraphPush listed in Table~\ref{tbl:comparison} in the original manuscript is incorrect. We sincerely thank the reviewer for pointing out this typo, and we are sorry for this discrepancy. We have corrected this typo in the revised paper. Please refer to Table~\ref{tbl:comparison} for details (also shown in Table~\ref{tbl:comparison_rev} given in the response letter for convenience). 

To see the superiority of our \setpush over the \sublinear method, recall that the expected time complexity of our \setpush is $\tilde{O}\left(\min \left\{d_t, \sqrt{m}\right\}\right)$. If $d_t \ge \sqrt{m}$, then our \setpush improves the \sublinear method by a factor of: 
\begin{align*}
\frac{\min\left\{\hspace{-0.5mm}\frac{m^{\frac{2}{3}} d^{1/3}_{max}}{d^{\frac{2}{3}}}, \frac{m^{\frac{4}{5}}}{d^{\frac{3}{5}}}\hspace{-0.5mm}\right\}}{\min \left\{d_t, \sqrt{m}\right\}}\hspace{-0.5mm}=\hspace{-0.5mm}\min\left\{\hspace{-0.5mm}\frac{m^{\frac{2}{3}} d^{1/3}_{max}}{d^{\frac{2}{3}} m^{\frac{1}{2}}}, \frac{m^{\frac{4}{5}}}{d^{\frac{3}{5}} m^{\frac{1}{2}}}\hspace{-0.5mm}\right\} \hspace{-0.5mm}= \hspace{-0.5mm}\min\left\{\hspace{-0.5mm}\frac{n^{\frac{1}{6}} d_{\max}^{1/3}}{d^{\frac{1}{2}}}, \frac{n^{\frac{3}{10}}}{d^{\frac{3}{10}}}\hspace{-0.5mm}\right\}. 
\end{align*}
Otherwise (i.e., $d_t < \sqrt{m}$), \setpush improves \sublinear by a factor of: 
\begin{align*}
\frac{\min\left\{\hspace{-0.5mm}\frac{m^{\frac{2}{3}} d^{1/3}_{max}}{d^{\frac{2}{3}}}, \frac{m^{\frac{4}{5}}}{d^{\frac{3}{5}}}\hspace{-0.5mm}\right\}}{\min \left\{d_t, \sqrt{m}\right\}}
\hspace{-0.5mm}=\hspace{-0.5mm}\min\left\{\hspace{-0.5mm}\frac{m^{\frac{2}{3}} d^{1/3}_{max}}{d^{\frac{2}{3}} d_t}, \frac{m^{\frac{4}{5}}}{d^{\frac{3}{5}} d_t}\hspace{-0.5mm}\right\} 
\hspace{-0.5mm}= \hspace{-0.5mm}\min\left\{\hspace{-0.5mm}\frac{n^{\frac{2}{3}} d_{\max}^{1/3}}{d_t}, \frac{n^{\frac{3}{5}}d^{\frac{1}{5}}}{d_t}\hspace{-0.5mm}\right\}. 
\end{align*}
Consequently, we can derive that the improvement of \setpush over the \sublinear method is: 
\begin{align*}
\max \left\{\min \left\{\frac{n^{\frac{2}{3}}\cdot d_{\max}^{1/3}}{d_t}, \frac{n^{\frac{4}{5}} \cdot d^{\frac{1}{5}}}{d_t}\right\}, \min\left\{\frac{n^{\frac{1}{6}}\cdot d_{\max}^{1/3}}{d^{\frac{1}{2}}}, \frac{n^{\frac{3}{10}}}{d^{\frac{3}{10}}}\right\}\right\}\ge 1. 
\end{align*}
And the above inequality takes equation when $d=n$ (i.e., on a complete graph). We present a detailed illustration on the superiority of our \setpush over the \sublinear method in our response to D2 of Reviewer \#4. Please refer to those illustrations for details. 




\review{\bf D7}: {\em The computation of gound-truth PageRank values is discussed in the Experiments. But it is unclear how this is used in the experiments. Also, it would be better to also test the actual accuracy achieved by the tested algorithms. } 

\header{\bf Response: } {\rev TODO}





\review{\bf D9}: {\em Proofreading is needed for the paper. } 

\header{\bf Response: } We have corrected all these typos and made a careful proofreading of the paper. Thanks for pointing out this! 
